Mesorasi: Architecture Support for Point Cloud Analytics via Delayed-Aggregation

Point cloud analytics is poised to become a key workload on battery-powered embedded and mobile platforms in a wide range of emerging application domains, such as autonomous driving, robotics, and augmented reality, where efficiency is paramount. This paper proposes Mesorasi, an algorithm-architecture co-designed system that simultaneously improves the performance and energy efficiency of point cloud analytics while retaining its accuracy. Our extensive characterizations of state-of-the-art point cloud algorithms show that, while structurally reminiscent of convolutional neural networks (CNNs), point cloud algorithms exhibit inherent compute and memory inefficiencies due to the unique characteristics of point cloud data. We propose delayed-aggregation, a new algorithmic primitive for building efficient point cloud algorithms. Delayed-aggregation hides the performance bottlenecks and reduces the compute and memory redundancies by exploiting the approximately distributive property of key operations in point cloud algorithms. Delayed-aggregation let point cloud algorithms achieve 1.6x speedup and 51.1% energy reduction on a mobile GPU while retaining the accuracy (-0.9% loss to 1.2% gains). To maximize the algorithmic benefits, we propose minor extensions to contemporary CNN accelerators, which can be integrated into a mobile Systems-on-a-Chip (SoC) without modifying other SoC components. With additional hardware support, Mesorasi achieves up to 3.6x speedup.

==> Mesorasi_ Enabling Efficient Point Cloud Analytics via Delayed-Aggregation/abst.tex <==
\begin{abstract}

%While conventional visual algorithms operating on images and videos have been well-optimized, point cloud analytics require considerably different algorithms and are less understood. Through a systematic characterization of today's point cloud algorithms, we show that point cloud algorithms are inefficient on today's hardware architectures due to their inherent algorithmic characteristics.

Point cloud analytics is poised to become a key workload on battery-powered embedded and mobile platforms in a wide range of emerging application domains, such as autonomous driving, robotics, and augmented reality, where efficiency is paramount. This paper proposes \proj, an algorithm-architecture co-designed system that simultaneously improves the performance and energy efficiency of point cloud analytics while retaining its accuracy.

%While consisting of familiar building blocks such as neighbor search and multi-layer perceptron that have been well-optimized, today's point cloud algorithms expose unique memory and compute inefficiencies. 

Our extensive characterizations of state-of-the-art point cloud algorithms show that, while structurally reminiscent of convolutional neural networks (CNNs),  point cloud algorithms exhibit inherent compute and memory inefficiencies due to the unique characteristics of point cloud data. We propose \textit{delayed-aggregation}, a new algorithmic primitive for building efficient point cloud algorithms. Delayed-aggregation hides the performance bottlenecks and reduces the compute and memory redundancies by exploiting the \textit{approximately distributive} property of key operations in point cloud algorithms. Delayed-aggregation let point cloud algorithms achieve 1.6$\times$ speedup and 51.1\% energy reduction on a mobile GPU while retaining the accuracy (-0.9\% loss to 1.2\% gains). To maximize the algorithmic benefits, we propose minor extensions to contemporary CNN accelerators, which can be integrated into a mobile Systems-on-a-Chip (SoC) without modifying other SoC components. With additional hardware support, \proj achieves up to 3.6$\times$ speedup.

\end{abstract}

==> Mesorasi_ Enabling Efficient Point Cloud Analytics via Delayed-Aggregation/algo.tex <==
\section{Delayed-Aggregation Algorithm}
\label{sec:algo}

\begin{figure*}[t]
\centering
\begin{minipage}[t]{0.65\columnwidth}
  \centering
  \includegraphics[width=\columnwidth]{ops_reduction}
  \caption{MAC operation reduction in the MLP by delayed-aggregation. The MAC count reductions come from directly operating on the input points as opposed to aggregated neighbors.}
  \label{fig:overall_ops_red}
\end{minipage}
\hspace{5pt}
\begin{minipage}[t]{0.65\columnwidth}
  \centering
  \includegraphics[width=\columnwidth]{layer_ops}
  \caption{Layer output size distribution as a violin plot with and without delayed-aggregation. High and low ticks denote the largest and smallest layer outputs, respectively.}
  \label{fig:layer_mem_red}
\end{minipage}
\hspace{5pt}
\begin{minipage}[t]{0.65\columnwidth}
  \centering
  \includegraphics[width=\columnwidth]{pointnet_dist}
  \caption{Time distribution across $\cN$, $\cA$, and $\cF$ in PointNet++ (s) with and without delayed-aggregation. Note that delayed-aggregation would also allow $\cN$ and $\cF$ to be executed in parallel.}
  \label{fig:pointnet_dist}
\end{minipage}
\end{figure*}

We introduce delayed-aggregation, a  primitive for building efficient point cloud networks (\Sect{sec:algo:algo}). Delayed-aggregation improves the compute and memory efficiencies of point cloud networks without degrading accuracy (\Sect{sec:algo:eff}). We show that aggregation emerges as a new bottleneck in new networks, motivating dedicated hardware support (\Sect{sec:algo:bn}).

%We show that our new algorithm approximates the existing algorithm with approximation introduced only by the non-linearity in MLPs. With re-training and/or fine-tuning, the new algorithm could match, sometimes even outperform, the accuracy of original algorithm.

%This section first describes a XXX algorithm to exploit the reuse (\Sect{sec:algo:algo}) and eliminate computation redundancy. We then demonstrate the performance gap (\Sect{sec:algo:speedup}) between static analysis and runtime measurement, which reveals the limitation of pure algorithm and the demand for hardware support. (\Sect{sec:algo:hw_motivation}).

\subsection{Algorithm}
\label{sec:algo:algo}

%Point cloud modules extract local features of a point by aggregating the point with its neighbors. The aggregation happens \textit{before} feature extraction ($\cF$). Early aggregation leads to two fundamental inefficiencies. First, it serializes neighbor search ($\cN$) with feature extraction, increasing the critical path latency as both $\cN$ and $\cF$ contribute to non-trivial execution time (\Fig{fig:motivation-dist}). Second, feature extraction leads to excessive irregular memory traffic (\Fig{fig:xx}). This is because the same input point is normalized to different values in different neighborhoods, preventing data reuse.

We propose a new framework for building efficient point cloud algorithms. The central idea is to delay aggregation until \textit{after} feature computation so that features are extracted on individual input points rather than on aggregated neighbors. Delayed-aggregation has two benefits. First, it allows neighbor search and feature computation, the two time-consuming components, to be executed in parallel. Second, feature computation operates on input points rather than aggregated neighbors, reducing the compute and memory costs.

%The new algorithm aggregates neighbors in the output feature space rather than in the input feature space as in the original algorithm.

\paragraph{Delayed-Aggregation} The key insight is that feature extraction ($\cF$) is \textit{approximately distributive} over aggregation ($\cA$). For an input point $\mathbf{p}_i$ and its corresponding output $\mathbf{p}_o$:

\begin{align}
  \mathbf{p}_o = \cF(\cA(\cN(\mathbf{p}_i),~~\mathbf{p}_i)) \approx \cA(\cF(\cN(\mathbf{p}_i)),~\cF(\mathbf{p}_i))
  \label{eq:fdist}
\end{align}

Fundamentally, \Equ{eq:fdist} holds because the MLP in $\cF$ is approximately distributive over subtraction in $\cA$. Specifically, applying an MLP to the difference of two matrices is approximately equivalent to applying an MLP to both matrices and then subtract the two resulting matrices. The approximation is introduced by the non-linearity in the MLP (e.g., ReLU):

\begin{align}
	& \phi(\phi(
	\begin{bmatrix}
	\mathbf{p}_1 - \mathbf{p}_i \\
	... \\
	\mathbf{p}_k - \mathbf{p}_i
	\end{bmatrix}
	\times W_1) \times W_2) \approx \nonumber \\
	& \phi(\phi(
	\begin{bmatrix}
	\mathbf{p}_1 \\
	... \\
	\mathbf{p}_k
	\end{bmatrix}
	\times W_1 \times W_2)) - \phi(\phi(
	\begin{bmatrix}
	\mathbf{p}_i \\
	... \\
	\mathbf{p}_i
	\end{bmatrix}
	\times W_1 \times W_2))
	\label{eq:mlpdist}
\end{align}

\noindent where $\mathbf{p}_1, ..., \mathbf{p}_k$ are neighbors of $\mathbf{p}_i$, $W_1$ and $W_2$ are the two weight matrices in the MLP (assuming one hidden layer), and $\phi$ is the non-linear activation function. Without $\phi$, the distribution of MLP over subtraction is precise. In actual implementation, the computation on $[\mathbf{p}_i~~...~~\mathbf{p}_i]^\intercal$ is simplified to operating on $\mathbf{p}_i$ once and scattering the result $K$ times.

Critically, applying this distribution allows us to decouple $\cN$ with $\cF$. As shown in \Equ{eq:fdist} and \Equ{eq:mlpdist}, $\cF$ now operates on original input points, i.e., $\mathbf{p}_i$ and $\cN({\mathbf{p}_i})$ (a subset of the input points, too) rather than the normalized point values ($\mathbf{p}_k - \mathbf{p}_i$), which requires neighbor search results. As a result, we could first apply feature computation on all input points. The computed features are then aggregated later.

\paragraph{Walk-Through} We use the first module in PointNet++ as an example to walk through the new algorithm. This module consumes 1024 ($N_{in}$) input points, among which 512 undergo neighbor search. Thus, the module produces 512 ($N_{out}$) output points. The input feature dimension is 3 ($M_{in}$) and the output feature dimension is 128 ($M_{out}$). \Fig{fig:newalgo} shows this module implemented with delayed-aggregation.

We first compute features ($\cF$) from all 1024 points in the input point cloud and store the results in the Point Feature Table (PFT), a $1024 \times 128$ matrix. Every PFT entry contains the feature vector of an input point. Meanwhile, neighbor searches ($\cN$) are executed in parallel on the input point cloud, each returning 32 neighbors of a centroid. The results of neighbor search are stored in a Neighbor Index Table (NIT), a $512 \times 32$ matrix. Each NIT entry contains the neighbor indices of an input point. In the end, the aggregation operation ($\cA$) aggregates features in the PFT using the neighbor information in the NIT. Note that it is the features that are being aggregated, not the original points.
%Effectively, the aggregation is delayed after the feature extraction.

Each aggregated matrix ($32 \times 128$) is reduced to the final feature vector ($1 \times 128$) of an output point. If reduction is implemented by a max operation as is the common case, aggregation could further be delayed after reduction because subtraction is distributive over max: $max(\mathbf{p}_1 - \mathbf{p}_i, \mathbf{p}_2 - \mathbf{p}_i) = max(\mathbf{p}_1, \mathbf{p}_2) - \mathbf{p}_i$. This optimization avoids scattering $\mathbf{p}_i$, reduces the subtraction cost, and is mathematically precise.

%\paragraph{Accuracy} Delayed-aggregation is designed to be a primitive for building point cloud algorithms. We find that the training process overcomes the accuracy loss introduced by approximation. New algorithms built with delayed-aggregation sometimes even out-perform the original algorithms (\Sect{sec:eval:acc}).
%It is possible to use delayed-aggregation as a runtime optimization without re-training. We find that the accuracy is generally lower.

\subsection{First-Order Efficiency Analysis}
\label{sec:algo:eff}

Compared with the original implementation of the same module in \Fig{fig:baselinealgo}, the delayed-aggregation algorithm provides three benefits. First, neighbor search and the MLP are now executed in parallel, hiding the latencies of the slower path.

%This is because the MLP directly operates on the input points. 
Second, we significantly reduce the MAC operations in the MLP. In this module, the original algorithm executes MLP on 512 $32 \times 3$ matrices while the new algorithm executes MLP only on one $1024 \times 3$ matrix. \Fig{fig:overall_ops_red} shows the MAC operation reductions across all five networks. On average, delayed-aggregation reduces the MAC counts by 68\%.

Third, delayed-aggregation also reduces the memory traffic because the MLP input is much smaller. While the actual memory traffic reduction is tied to the hardware architecture, as a first-order estimation \Fig{fig:layer_mem_red} compares the distribution of per-layer output size with and without delayed-aggregation. The data is shown as a violin plot. Delayed-aggregation reduces the layer output sizes from 8 MB\textasciitilde 32 MB to 512 KB\textasciitilde 1 MB, amenable to be buffered completely on-chip.
%, where the high and low ticks represent the largest and smallest layer output size, respectively, and the width of the violin represents the density at a particular size value ($y$-axis)

By directly extracting features from the input points, our algorithm unlocks the inherent data reuse opportunities in point cloud. Specifically in this example, \texttt{P3} is a neighbor of both \texttt{\underline{P1}} and \texttt{\underline{P2}}, but could not be reused in feature computation by the original algorithm because \texttt{P3}'s normalized values with respect to \texttt{\underline{P1}} and \texttt{\underline{P2}} are different. In contrast, the MLP in our algorithm directly operates on \texttt{P1}, whose feature is then reused in aggregation, \textit{implicitly} reusing \texttt{P1}.

\subsection{Bottleneck Analysis}
\label{sec:algo:bn}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{runtime_dist}
    \caption{Both absolute (left $y$-axis) and relative (right $y$-axis) aggregation times increase with delayed-aggregation.}
    \label{fig:runtime_dist}
\end{figure}

While delayed-aggregation reduces the compute costs and memory accesses, it also significantly increases the aggregation time. Using PointNet++ as an example, \Fig{fig:pointnet_dist} compares the execution time distribution across the three operations ($\cN$, $\cA$, and $\cF$) with and without delayed-aggregation. The error bars denote one standard deviation in the measurement. The feature extraction time significantly decreases, and the neighbor search time roughly stays the same --- both are expected. The aggregation time, however, significantly increases.
%Aggregation is now the roadblock to fully unleashing the potential of delayed-aggregation.

\Fig{fig:runtime_dist} generalizes the conclusion across the five networks. The figure compares the absolute (left $y$-axis) and relative (right $y$-axis) aggregation time in the original and new algorithms. The aggregation time consistently increases in all five networks. Since neighbor search and feature computation are now executed in parallel, aggregation overhead contributes even more significantly to the overall execution time. On average, the aggregation time increases from 3\% to 24\%.

Aggregation time increases mainly because aggregation involves irregular gather operations~\cite{kirk2016programming}, which now operate on a much larger working set with delayed-aggregation. For instance, in PointNet++'s first module (\Fig{fig:newalgo}), aggregation originally gathers from a 12 KB matrix but now gathers from a 512 KB matrix, which is much larger than the L1 cache size (48 KB -- 96 KB\footnote{To our best knowledge, Nvidia does not publish the L1 cache size for the mobile Pascal GPU in TX2 (GP10B~\cite{gp10b}). We estimate the size based on the L1 cache size per SM in other Pascal GPU chips~\cite{pascaluarch} and the number of SMs in the mobile Pascal GPU~\cite{tx2spec}}) in the mobile Pascal GPU on TX2.

The working set size increases significantly because aggregation in new algorithms gathers data from the PFT, whose dimension is $N_{in} \times M_{out}$, whereas the original algorithms gather data from the input point matrix, whose dimension is $N_{in} \times M_{in}$. $M_{out}$ is usually several times greater than $M_{in}$ in order to extract higher-dimensional features. In the example above, $M_{out}$ is 128-D whereas $M_{in}$ is 3-D.

%While the delayed-aggregation enables the MLP processing on individual points instead of their neighbors to reduce the computations, the aggregation that operating on higher dimensional feature vectors incurs overheads on memory access. To understand the efficacy of the new algorithm, we first analyze the theoretical improvements of MAC operations and overall speedup, and we then characterize the variation of every operation that brought by delayed-aggregation.

%The delayed aggregation decouples the neighbors from feature extraction in MLP, which brings computation efficiency by reducing the input data from aggregated neighbors to individual points. Intuitively, it can achieve \textit{K} times of computation reduction, where \textit{K} is the number of a point's neighbors.

%We calculate the MAC operations in MLP with the size of the intermediate feature map, as it directly reflects the number of computations. Given the reduction of computations and the time that MLP dominates in an algorithm, we then estimate the overall speedup. Comparing with the original algorithm, \Fig{} shows that we have the potential to reduce about \fixme{XX\% - XX\%} of MAC operations and achieve \fixme{aaX - bbX} speedup.

%The new algorithm brings not only improvements on MLP but also overheads in aggregation, therefore, we go in-depth to examine the effect of delaying aggregation on every single operation. Under the same environment that used for the characterization in \Sect{}, we implement the new algorithm and collect the total execution time of each operation. 

%\Fig{} shows the operation-wise comparison between the old and new \fixme{FPointNet++} algorithm. The time spend on MLP is significantly reduced as expected, and most of the other operations spend less or similar time due to the reduced data size. However, the extra overhead on aggregation is confirmed to be unignorable and critical. 

%We show only the detailed breakdown data for one DNN algorithm as an example, and we further test on all other algorithms to solidify this conclusion. \Fig{} highlights the speedup of MLP and aggregation, where all other trivial operations are lumped together.

% % \subsection{The Need for Hardware Support}
% \label{sec:algo:speedup}
% Benefit from the decoupling between neighbors and centroids, the simplified computations in MLP are related to the number of input points only instead of the number of their neighbors. To fully understand the efficacy of the new algorithm, we first calculate the theoretic speedup statically and then measure the practical runtime. We observe that there is a performance gap between theory and practice that calls for the hardware support, and we finally locate the exact target that demands acceleration.


% % \paragraph{Savings}


% \paragraph{Gap Between Theory and Practical}
% The performance improvement of the XXX algorithm comes from both reduced computations and memory traffic in MLP. To simplify the analysis, we ignore the profit brought by memory traffic and estimate a conservative overall speedup with the reduced Multiply-Accumulate (MAC) Operations.

% Our estimation follows the Amdahl's law, where the percentage of MLP execution time in a DNN algorithm comes from the distribution data in \Sect{}, and the speedup for MLP is determined by the Downsample parameter and the total number of a centroid's neighbors. Assume 1024 points with $<x, y, z>$ coordinates are sampled as 512 centroids, and each centroid has 32 neighbors. The size of input data to the MLP is $(512\times32)\times3$ and $1024\times3$ values on the original and decoupled algorithm, respectively. The number of weights and bias of MLP only related to the structure of the MLP itself, which results in the reduction of MAC operations equivalent to the reduction of input data size (i.e., 16X in this example).

% To obtain the real overall speedup, we implement the XXX algorithm in the same environment that used for characterization in \Sect{}. We then measure the total execution time of XXX algorithm and compute the speedup over the original algorithms. 

%\begin{figure}[t]
%%\vspace{-10pt}
%    \centering
%    \captionsetup[subfigure]{width=0.47\columnwidth}
%	\subfloat[.]
%	% conducted by choosing the $k^{th}$ closest neighbor.
%	{
%  		\label{fig:speedup_overall}
%  		\includegraphics[width=0.47\linewidth]{speedup_overall}
%	}\hfill
%	\subfloat[.]
%	% conducted by substituting the actual results with points within the specified spherical range.
%	{
%  		\label{fig:speedup_component}
%  		\includegraphics[width=0.47\linewidth]{speedup_overall}
%	}
%	\vspace{-10pt}
%	\subfloat[.]
%	% conducted by substituting the actual results with points within the specified spherical range.
%	{
%  		\label{fig:component_breakdown}
%  		\includegraphics[width=0.95\linewidth]{component_breakdown}
%	}
%	\vspace{-10pt}
%    \caption{Pseudo Figure.}
%    %\vspace{-5pt}
%\end{figure}

% \Fig{} shows the comparison between estimated and measured speedup, and the evaluation runs on 6 DNN algorithms from 3 representative deep learning tasks: classification, segmentation, and object detection. We observe a significant performance gap between XXX and the original algorithm, which thus leads to a detailed analysis of the root causes.  

% \paragraph{Root Causes}
% The decoupled XXX algorithm postpones the Grouping and Normalization to the end of the PCM, which shrinks the size of input data to MLP but incurs overhead in recoupling, as the Grouping and Normalization operate on point's feature vector instead of raw coordinates.

% With the same parameter set we illustrate before, the MLP saves the MAC operations from $(512\times32)\times3$ to $1024\times3$, while the total element for Grouping to access increases from $512\times32\times3$ to $512\times32\times128$. Normalization as a pointwise operation, it supposes to increase the same number of MAC operations as the Grouping's accesses, but the redundancy-free design in BE reduces the operations from $512\times32\times128$ to $512\times1\times128$.

% Intuitively, there is a trade-off between the savings in MLP and the overheads in the recoupling. To quantitively understand the costs and benefits, we re-profile the XXX algorithm and compare against the original algorithms in \Sect{} with the identical experiment configurations.

% We compare the time breakdown between XXX and the original algorithms in \Fig{}, where the time spends on MLP and recoupling are highlighted and the rest components are lumped together. While the decoupled XXX algorithm reduces the time consumption on MLP, the overheads in recoupling are one candidate that diminish the benefits. To exhaustively examine whether there are other overheads, we further breakdown the single operations within a DNN algorithm. We show only one example in \Fig{}, which confirms that only Grouping incurs considerable overheads.

%The XXX algorithm exposes the opportunities for exploiting data/computation reuse, redundancy elimination, and parallelism, \fixme{with cost of intensive memory accesses}. Our quantitive analyzation proves the efficacy of the decoupling design, but also reveals the pure software implementation is incapable to alleviate the overhead.

% 
% \subsection{Inefficiency Discussion}
% \label{sec:algo:hw_motivation}
% The goal is to focus on the problems that cannot be addressed by software changes. \\

% % \subsection{On-chip Memory Scheduling}
% % \fixme{we should decide where to put this section, here or later in the architecture part.} \\
% % Space-filling curve.  The new pipeline postpones the irregular memory access from the beginning to the end of the MLP computations, but itself does not alleviate the irregularities. I assume that we still need the space-filling curve to capture the locality, and I feel it would be better to integrate into the vanilla software pipelines and claim that the construction of the KD-tree search inherently provides such information.

% Here we provide the breakdown of total execution time for both baseline and our new design. We could also show the speed up on MLPs and other components to claim that the gain on the MLP part is as expected, while the time spent on other parts becomes dominant in our software design.

%     Software limitations can be classified into two aspects. 

%     \begin{itemize}
%       \item (1) point cloud-specific (find neighbors, grouping and sampling)
%       \item (2) conventional components (BN, bias add)
%     \end{itemize}

%     Limitation (1) pave the way for us to introduce the neighbor search engine in the next section. The existing optimizations do not work on these parts, which motivates novel architecture support. 

%     Limitation (2) expose the performance issue on those conventional components. Depends on our hardware design, the way we explain it might be different. For example, if we want to have a TPU-like design for MMM, then the BN here might introduce synchronization cost, and thus we might want to get rid of it. Or if we want to have some hardware for BN, it also motivates the design. (I guess people ignores the optimization on BN in conventional NNs probable due to the time spent on BN is negligible, which however is not the case for point cloud DNNs)

% At the end of this section, we claim that even though we parallel the new pipeline, the whole system is still under-optimized and demands hardware supports.


==> Mesorasi_ Enabling Efficient Point Cloud Analytics via Delayed-Aggregation/arch.tex <==
\section{Architectural Support}
\label{sec:arch}

%1). Specialized compute engines for different operations, e.g., neighbor search, sampling, MLPs;
%2). How do different compute units coordinate;
%3). On-chip memory scheduling strategies;

\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{soc}
%\vspace{-5pt}
\caption{The \proj SoC builds on top of today's SoCs consisting of a GPU and a DNN accelerator (NPU). Neighbor search executes on the GPU and feature extraction executes on the NPU. \proj augments the NPU with an aggregation unit (AU) to efficiently execute the aggregation operation. The AU structures are shaded (colored).}
\label{fig:soc}
\end{figure}
%Our design is independent of where the non-MLP part is executed, which could be on a GPU or a dedicated neighbor search engine (NSE).

\begin{figure*}[t]
\centering
\includegraphics[width=2.1\columnwidth]{grouping}
\caption{Aggregation unit. The NIT buffer is double-buffered from the DRAM. The Address Generation logic simply fetches addresses already buffered in the NIT and sends them to the PFT buffer controller. The PFT buffer is organized as B independently addressed single-ported SRAMs. It could be thought of as an optimized version of a traditional B-banked, B-ported SRAM, because it does not need the crossbar that routes data from banks to ports (but does need the crossbar to route an address to the corresponding bank). The PFT buffer is connected to the NPU's global buffer. Each bank produces one word (Wr) per cycle. The shift registers hold up to $M_{out}$ words, where $M_{out}$ is the output feature vector size. The top shift register holds the result of reduction, and the bottom shift register holds the feature vector of a centroid.}
\label{fig:groupinghw}
%\vspace{-5pt}
\end{figure*}

This section describes \proj, our hardware design that efficiently executes point cloud algorithms developed using delayed-aggregation. \proj extends existing DNN accelerators with minor augmentations while leaving the rest of the SoC untouched. We start from an overview of \proj and its workflow (\Sect{sec:arch:ov}), followed by a detailed description of the architecture support (\Sect{sec:arch:aug}).
% and design decision discussions (\Sect{sec:arch:des}).

\subsection{Overall Design}
\label{sec:arch:ov}

%We first describe how the point cloud algorithms are executed on today's SoCs, and then introduce our architectural augmentations that enable an efficient execution of our proposed algorithms.
We assume a baseline SoC that incorporates a GPU and an NPU, as with emerging mobile SoCs such as Nvidia Xavier~\cite{xaviersoc}, Apple A13~\cite{applea13}, and Microsoft HPU~\cite{hpuaicore}. Point cloud algorithms are a few times faster when an NPU is available to accelerate MLP compared to running only on the GPU (\Sect{sec:eval:res}). Thus, an NPU-enabled SoC represents the trend of the industry and is a more optimized baseline.

\paragraph{Design} \Fig{fig:soc} shows how \proj augments the NPU in a generic SoC. In \proj, the GPU executes neighbor search ($\cN$) and the NPU executes feature extraction ($\cF$), i.e., the MLP. In addition, \proj augments the NPU with an Aggregation Unit (AU) to efficiently execute the aggregation operation ($\cA$). As shown in \Sect{sec:algo:bn}, aggregation becomes a bottleneck in our new algorithms and is inefficient on the GPU. AU minimally extends a generic NPU architecture with a set of principled memory structures and datapaths.
%AU does not rely on a specific NPU architecture. Instead, 

%\proj does not rely on a particular NPU architecture, and requires minor and principled changes to the NPU architecture as we will discuss later.

%However, \proj makes no assumption about the actual neighbor search algorithm. Some point cloud pipelines use a KD-tree based search algorithm whereas others use exhaustive distance computation combined with top-K selection~\cite{??}; both have efficient GPU implementations~\cite{??}.
\proj maps $\cN$ to the GPU because neighbor search is highly parallel, but does not map to the specialized datapath of an NPU. Alternatively, an SoC could use a dedicated neighbor search engine (NSE)~\cite{Kuhara2013An, xu2019tigris}. We use the GPU because it is prevalent in today's SoCs and thus provides a concrete context to describe our design. We later show that delayed-aggregation could achieve even higher speedups in a futurist SoC where an NSE is available to accelerate neighbor search (\Sect{sec:eval:nse}). In either case, \proj does not modify the internals of the GPU or the NSE.
%\proj augmentations are independent of where non-MLP operations are executed, but we assume that they execute on a GPU in order to provide a concrete context to describe our design.

%While it is possible to use only the GPU for the entire point cloud execution, as with the profiling experiments presented before, using an NPU provides a stronger baseline and thus does not unfairly favor our proposal.

%The CPU coordinates the GPU and the DNN accelerator, whose tasks must be serialized in the original point cloud algorithms. Specifically, once the GPU finishes the neighbor search and grouping, the grouped matrices, which will become the input feature maps to the MLP layers, are stored back to the DRAM. The CPU then triggers the DNN accelerator to read the input feature maps to execute the MLP layers and produce the output.

%The rationale for this baseline is to construct the best baseline so as to not unfairly favor our proposal. The MLPs are most efficient on a dedicated accelerator. The KNN search and grouping operations are inherently parallel, but do not fit on the DNN accelerator. Transferring them back to the CPU would require lots of data movement and are inefficient.

\paragraph{Work Flow} Point cloud algorithms with delayed-aggregation work on \proj as follows. The input point cloud is initially stored in the DRAM. The CPU configures and triggers the GPU and the NPU simultaneously, both of which read the input point cloud. The GPU executes the KNN search and generates the Neighbor Index Table (NIT), which gets stored back to the DRAM. Meanwhile, the NPU computes features for input points and generates the Point Feature Table (PFT). The AU in NPU combines the PFT with the NIT from the memory for aggregation and reduction, and eventually generates the output of the current module.

In some algorithms (e.g., PointNet++), neighbor searches in all modules search in the original 3-D coordinate space, while in other algorithms (e.g., DGCNN) the neighbor search in module $i$ searches in the output feature space of module ($i-1$). In the latter case, the current module's output is written back to the memory for the GPU to read in the next module.
%In both cases, the current module output is reused by the NPU for feature extraction in the next module.

%Our new algorithm framework allows KNN search and MLP layers to be decoupled and executed in parallel. With MLP redundancies greatly reduced (\fixme{100}$\times$, see~\Sect{sec:xx}) and the KNN search decoupled, we find that the group operations becomes the bottleneck. The grouping operation is inefficient on GPU because it requires irregular memory accesses (\Fig{fig:nsreuse}). \fixme{needs data.}

%Our design augments the DNN accelerator to execute the group operation as shown in~\Fig{fig:soc}. The architectural augmentation employs specialized memory structures and datapaths design to improve the memory access efficiency in grouping. In doing this, the point feature table could also directly be reused on-chip within the NPU without having to be transferred by the GPU.

Our design modifies only the NPU while leaving other SoC components untouched. This design maintains the modularity of existing SoCs, broadening the applicability. We now describe the AU augmentation in NPU in detail.

%we propose two principled modifications to the baseline SoC architecture. First, we allow the GPU and the DNN accelerator to execute in parallel. This is achieved through a single control logic (finite-state machine), which sets the memory mapped registers in both IP blocks to trigger them.

%Second, we add a small, dedicated piece of SRAM on-chip to hold the results of the neighbor search, i.e., the neighbor index table (NIT). The GPU writes the result of neighbor search to NIT. NIT is not needed in the baseline, where the group operation is executed on the GPU.

%Finally, we propose a new grouping unit (GU), which is decoupled from GPU. Grouping contributes significantly to the baseline software implementation because it requires large chunk of irregular memory accesses that leads to high bank conflict on GPUs. The GU uses specialized memory structures to speedup the group operation. The GU reads the output matrix from the MLP layers, and generates the matrices that will then be used by the max pooling unit to generate the output of a module.

\subsection{Aggregation Unit in NPU}
\label{sec:arch:aug}

Aggregation requires irregular gather operations that are inefficient on GPUs. The key to our architectural support is the specialized memory structures co-designed with customized data structure partitioning, which provide efficient data accesses for aggregation with a little area overhead.

Algorithmically, aggregation iterates over the NIT's $N_{out}$ entries until NIT is exhausted. Each NIT entry contains the $K$ neighbor indices of a centroid $\mathbf{p}$. The aggregation operation first gathers the $K$ corresponding entries (feature vectors) from the PFT ($N_{in} \times M_{out}$). The $K$ feature vectors are then reduced to one ($1 \times M_{out}$) vector, which subtracts $\mathbf{p}$'s feature vector to generate the output feature for $\mathbf{p}$.
% Once all $N_{out}$ entries are finished, a $N_{out} \times M_{out}$ matrix is generated, which is used in the next module.

\Fig{fig:groupinghw} shows the detailed design of the aggregation unit. The NIT is stored in an SRAM, which is doubled-buffered in order to limit the on-chip memory size. The PFT is stored in a separate on-chip SRAM connected to the NPU's global buffer (which stores the MLP weights and input/output). This allows the output of feature extraction to be directly transferred to the PFT buffer without going through the DRAM. Similarly, the aggregation output is directly written back to the NPU's global buffer, as the aggregation output of the current module is the input to the feature extraction in the next module.

To process each NIT entry, the Address Generation Unit (AGU) uses the $K$ indices to generate $K$ addresses to index into the PFT buffer. Due to the large read bandwidth requirement, the PFT buffer is divided into $B$ independently addressable banks, each of which produces 1 word per cycle.
% (4 bytes in \proj).
% as we use the single precision data format).

Each cycle, the PFT buffer produces $B$ words, which enters the reduction unit. In our current design, the reduction unit implements the max logic as is the case in today's point cloud algorithms. The output of the max unit, i.e., the max of the $B$ words, enters a shift register (the top one in \Fig{fig:groupinghw}). Ideally, the number of banks $B$ is the same as the number of neighbors $K$ and the $K$ addresses fall into different banks. If so, the shift register is populated with the $1 \times M_{out}$ vector after $M_{out}$ cycles. The AGU then reads $\mathbf{p}$'s feature vector from the PFT buffer and stores it in another shift register (the bottom one in \Fig{fig:groupinghw}). The two shift registers perform an element-wise subtraction as required by aggregation. The same process continues until the entire NIT is exhausted.

%, in which case only a subset of the $B$ banks produces meaningful data each cycle
\paragraph{Multi-Round Grouping} In reality, reading the neighbor feature vectors takes more than $M_{out}$ cycles because of two reasons. First, $K$ could be greater than $B$. The number of banks $B$ is limited by the peripheral circuits overhead, which increases as $B$ increases. Second, some of the $K$ addresses could fall into the same bank, causing bank conflicts. We empirically find that an LSB-interleaving reduces bank conflicts, but it is impossible to completely avoid bank conflict at runtime, because the data access patterns in point cloud are irregular and could not be statically calculated -- unlike conventional DNNs and other regular kernels.
%Banks that do not output useful words toggle a flag, indicating its output should be ignored by the MaxPooling unit. 

We use a simple multi-round design to handle both non-ideal scenarios. Each round the AGU would attempt to identify as many unconflicted addresses as possible, which is achieved by the AGU logic examining each address modulo $B$. The unconflicted addresses are issued to the PFT buffer, whose output enters the max unit to generate a temporary output stored in the shift register. The data in the shift register would be combined with the PFT output in the next round for reduction. This process continues until all the addresses in an NIT buffer entry are processed.

An alternative way to resolve bank-conflict would be to simply ignore conflicted banks, essentially approximating the aggregation operation. We leave it to future work to explore this optimization and its impact on the overall accuracy.

%\paragraph{Optimizing for Bank Conflicts} We leverage a unique algorithmic characteristics in point cloud algorithms to reduce bank conflict. Many point cloud algorithms such as PointNet++~\cite{??} identify $K$ neighbors of a centroid by returning $K$ arbitrary neighbors within a certain range. In cases where fewer than $K$ actual neighbors are found, the actual neighbors are duplicated to fill the $K$ neighbors. Accessing the duplicated neighbors would inevitably, but unnecessarily, result in bank conflicts.

\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{colpart}
%\vspace{-5pt}
\caption{Column-major partitioning of PFT to reduce PFT buffer size (4 partitions in this example). Each time the PFT buffer is filled with only one partition. Since reduction (max) is applied to each column independently, the column-major partitioning ensures that all the neighbors of a centroid are present in the PFT buffer for aggregation.}
\label{fig:colpart}
\end{figure}

%\begin{figure*}[t]
%%\vspace{-10pt}
%\centering
%\subfloat[\small{Row-major partitioning. Each partition contains several PFT rows.}]
%{
%  \includegraphics[trim=0 0 0 0, clip, width=0.98\columnwidth]{rowpart}
%  \label{fig:rowpart}
%}
%\hspace{5pt}
%\subfloat[\small{Column-major partitioning.  Each partition contains several PFT columns.}]
%{
%  \includegraphics[trim=0 0 0 0, clip, width=0.98\columnwidth]{colpart}
%  \label{fig:colpart}
%}
%\caption{Partitioning PFT to reduce the PFT buffer size (4 partitions in this example). Each time the PFT buffer contains only one PFT partition. While requiring the same PFT buffer size, column-major partitioning is better than row-major partitioning. This is because reduction (max) is applied to each column independently; thus, the column-major partitioning ensures that all the neighbors of a centroid are present in the PFT buffer for aggregation.}
%\label{fig:partition}
%\end{figure*}

\paragraph{PFT Buffer Design} One could think of the PFT buffer as a $B$-banked, $B$-ported SRAM. Traditionally, heavily ported and banked SRAMs are area inefficient due to the crossbar that routes each bank's output to the corresponding issuing port~\cite{weste2015cmos}. However, our PFT buffer is much simplified \textit{without} the crossbar. This is by leveraging a key observation that the outputs of all the PFT banks are consumed by the max unit, which executes a \textit{commutative} operation, i.e., $max(a, b)=max(b, a)$. Thus, the output of each bank need not be routed to the issuing port so long as the requested data is correctly produced. This design optimization greatly reduces the area overhead (\Sect{sec:eval:area}).

One might be tempted to reuse the NPU's global buffer for the PFT buffer to save chip area. After all, the PFT \textit{is} MLP's output, which is stored in the global buffer. However, physically sharing the two SRAM structures is difficult, mainly because of their different design requirements. Global buffer contains MLP weights and layer inputs, accesses to which have regular patterns. As a result, NPU global buffers are usually designed with very few ports (e.g., one)~\cite{jouppi2017datacenter, armmlproc} while using a wide word. In contrast, accesses to the PFT are irregular as the neighbors of a centroid could be arbitrary spread in the PFT. Thus, the PFT buffer must be heavily-ported in order to sustain a high bandwidth requirement.

\paragraph{PFT Partitioning} To hold the entire PFT, the buffer must hold $N_{out} \times M_{out}$ features, which could be as large as 0.75~MB in some networks (e.g., DGCNN). Since the PFT buffer adds area overhead, we would like to minimize its size.

We partition the PFT to reduce the PFT buffer size. Each time, the PFT buffer is filled with only one partition. One straightforward strategy is the row-major partitioning, where the PFT buffer holds only a few rows of the PFT. However, since a centroid's neighbors could be arbitrarily spread across different PFT rows, row-major partitioning does not guarantee that all the neighbors of a centroid are present in the PFT buffer (i.e., in the same partition) for aggregation.

Instead, our design partitions the PFT column-wise, where each partition contains several columns of the PFT. \Fig{fig:colpart} illustrates the idea with 4 partitions. In this way, aggregation of a centroid is divided into four steps, each step aggregating only one partition. The column-major partitioning ensures that, within each partition, the neighbors of a centroid are available in the PFT buffer. Since reductions (max) of different columns are independent, the four intermediate reduction results can simply be concatenated in the end.

% we can also double-buffer the PFT buffer now with column-major partitioning. as we aggregate the current partition, the next partition can be loaded. this hides the latency to load PFT buffer.

With column-wise partitioning, each NIT entry is accessed multiples times---once per aggregation step. Thus, a smaller PFT buffer, while reducing the area overhead, would also increase the energy overhead. We later quantify this resource vs. energy trade-off (\Sect{sec:eval:sen}).

%\paragraph{Exploiting Locality} Different queries in the NIT have extensive data reuse due to the overlap across different neighbor searches, as illustrated in~\Fig{fig:nsreuse}. We propose to use a small fully-associative cache to exploit this locality. The cache stores the feature vectors for a small number of points and  avoids frequent accesses to the PFT buffer.
%
%To maximize the effectiveness of the cache, we reorder the queries in the NIT FIFO so as to improve the reuse across consecutive queries. While it is possible to scan all the FIFO entires to estimate the optimal order, it is inefficient and requires complex hardware design. Instead, we use the classic Z-order (Morton) space-filling curve heuristics~\cite{??} to reorder the FIFOs. Critically, the exact Z-order is inherently generated in neighbor search without requiring hardware modifications. Essentially, the natural order of the KD-tree leaf nodes is equivalent to the Z-order. Thus, we simply execute the KNN searches according to the Z-order, and the resulting order in the NIT is naturally Z-ordered. \fixme{more stuff}

%\subsection{Design Decisions}
%\label{sec:arch:des}

%\paragraph{Aggregation Scheduling} It is possible to better schedule the order of NIT entries in a way that maximize the 




















==> Mesorasi_ Enabling Efficient Point Cloud Analytics via Delayed-Aggregation/background.tex <==
\section{Background}
\label{sec:bck}

\paragraph{Point Cloud} A point cloud is an unordered set of points in the 3D Cartesian space. Each point is uniquely identified by its $<x$, $y$, $z>$ coordinates. While point cloud has long been used as a fundamental visual data representation in fields such as 3D modeling~\cite{alliez2017culture} and graphics rendering~\cite{gross2011point, levoy1985use, rusinkiewicz2000qsplat, pfister2000surfels}, it has recently received lots of attention in a range of emerging intelligent systems such as autonomous vehicles~\cite{geiger2012we}, robotics~\cite{whitty2010autonomous}, and AR/VR devices~\cite{stets2017visualization}.

\paragraph{Point Cloud Analytics} Similar to conventional visual analytics that analyzes images and videos, point cloud analytics distill semantics information from point clouds. Examples include object detection~\cite{geiger2012we}, semantics segmentation~\cite{behley2019semantickitti}, and classification~\cite{wu20153d}. While image and video analytics have been well-optimized, point cloud analytics require different algorithms and are much less optimized.

Point cloud algorithms operate by iteratively extracting features of each point. Conventional point cloud algorithms use ``hand-crafted'' features such as FPFH~\cite{rusu2009fast} and SHOT~\cite{tombari2010unique}. Recent deep learning-based algorithms use learned features and have generally out-performed conventional algorithms~\cite{chen2016eyeriss}. This paper thus focuses on deep learning-based algorithms.

We focus on deep learning-based algorithms that directly manipulate raw point clouds. Other data representations such as 2D projections of 3D points and voxelization suffer from low accuracy and/or consume excessively high memory~\cite{liu2019point}.





==> Mesorasi_ Enabling Efficient Point Cloud Analytics via Delayed-Aggregation/conc.tex <==
\section{Conclusion}
\label{sec:conc}

With the explosion of 3D sensing devices (e.g., LiDAR, stereo cameras), point cloud algorithms present exciting opportunities to transform the perception ability of future intelligent machines. \proj takes a systematic step toward efficient point cloud processing. The key to \proj is the delayed-aggregation primitive that decouples neighbor search with feature computation and significantly reduces the overall workload. Hardware support maximizes the effectiveness of delayed-aggregation. The potential gain is even greater in future SoCs where neighbor search is accelerated.

%We expect \proj to have a broad applicability to emerging problem domains such as autonomous vehicles, robotics, and Augmented/Virtual Reality, which all rely heavily on point cloud analytics.
%A key incentive for companies is that \proj not only provides significant speedup on GPUs, but also requires only very little and modular extension to conventional DNN accelerators, rather than being a new accelerator. The connection between point cloud analytics and GNNs suggest that some GNNs might also benefit from \proj, which we leave for future work.

==> Mesorasi_ Enabling Efficient Point Cloud Analytics via Delayed-Aggregation/eval.tex <==
\section{Evaluation}
\label{sec:eval}

We first show \proj adds little hardware overhead (\Sect{sec:eval:area}) while achieving comparable accuracy against original point cloud networks (\Sect{sec:eval:acc}). We then demonstrate the efficiency gains of \proj on different hardware platforms (\Sect{sec:eval:gpu} -- \Sect{sec:eval:nse}), followed by sensitivity studies (\Sect{sec:eval:sen}).

\subsection{Area Overhead}
\label{sec:eval:area}

\proj introduces only minimal area overhead with the minor AU augmentations. The main overhead comes from the 88 KB additional SRAM required for the PFT buffer and the NIT buffer. Compared to the baseline NPU, the additional hardware introduces less than 3.8\% area overhead (\SI{0.059}{\mm\squared}), which is even more negligible compared to the entire SoC area (e.g., \SI{350}{\mm\squared} for Nvidia Xavier~\cite{xaviersochotchips} and \SI{99}{\mm\squared} for Apple A13~\cite{applea13}).

Our custom-designed PFT buffer avoids the crossbar connecting the banks to the read ports by exploiting the algorithmic characteristics (\Sect{sec:arch:aug}). Since our PFT buffer is heavily banked (32) and ported (32) and each bank is small in size (2 KB), the additional area overhead introduced by the crossbar would have been high. Specifically, the area of the PFT buffer now is \SI{0.031}{\mm\squared}, but the crossbar area would be \SI{0.064}{\mm\squared}, which is now avoided.

\subsection{Accuracy}
\label{sec:eval:acc}

Overall, \proj matches or out-performs the original algorithms. We train all seven networks with delayed-aggregation from scratch until the accuracy converges. \Fig{fig:app_acc} compares our accuracy with that of the baseline models, which we choose the better of the reported accuracies in the original papers or accuracies from training their released code. Overall, \proj leads to at most 0.9\% accuracy loss in the case of PointNet++ (c) and up to 1.2\% accuracy gain in the case of F-PointNet. This shows that, while delayed-aggregation approximates the original algorithms, the accuracy loss could be recovered from training. Delayed-aggregation could be used as a primitive to build accurate point cloud algorithms.

We find that fine-tuning the model weights trained on the original networks has similar accuracies as retraining from scratch. However, directly using the original weights without retraining leads to a few percentages of accuracy loss, which is more significant when the non-linear layers use batch normalization, which perturbs the distributive property of matrix multiplication over subtraction more than ReLU.

\begin{figure}[t]
  %\vspace{-10pt}
  \centering
  \includegraphics[width=\columnwidth]{pcloud_accuracy}
  \caption{The accuracy comparison between networks trained with delayed-aggregation and the original networks.}
  \label{fig:app_acc}
  %\vspace{-10pt}
\end{figure}

% \begin{figure}[t]
%   %\vspace{-10pt}
%   \centering
%   \captionsetup[subfigure]{width=0.5\columnwidth}
%   \subfloat[\small{Overall Accuracy}]
%   {
%   \includegraphics[width=.48\columnwidth]{overall_cls_acc}
%   \label{fig:overall_cls_acc}
%   }
%   \subfloat[\small{Mean Class Accuracy}]
%   {
%   \includegraphics[width=.48\columnwidth]{mean_cls_acc}
%   \label{fig:mean_cls_acc}
%   }
%   %\vspace{-5pt}
%   \caption{Classification accuracy comparison between Original algorithms and accelerated algorithm.}
%   \label{fig:cls_acc}
%   %\vspace{-10pt}
% \end{figure}

%\paragraph{Object Classification} The first two columns in \Fig{fig:app_acc} show the comparison of overall classification accuracy between our \proj algorithms and their corresponding baselines. We applied our algorithmic acceleration on both PointNet++ and DGCNN. Overall, our \proj algorithms can achieve comparable accuracy against original baselines with an average \fixme{0.5\%} accuracy loss. Specifically, our accelerated algorithm achieves the same overall accuracy on DGCNN and >$1\%$ accuracy loss on PointNet++. This shows the generosity of our framework. Meanwhile, we also compared the mean class accuracy of both algorithms. The result shows that our \proj algorithm has \fixme{$1.7\%$} accuracy loss on PointNet++ and \fixme{$0.9\%$} accuracy loss on DGCNN. In \Sect{}, we show that the performance benefit of out accelerated algorithms wins over the slight accuracy loss.

% \begin{figure}[t]
%   %\vspace{-10pt}
%   \centering
%   \captionsetup[subfigure]{width=0.5\columnwidth}
%   \subfloat[\small{Overall Accuracy}]
%   {
%   \includegraphics[width=.48\columnwidth]{overall_seg_acc}
%   \label{fig:overall_seg_acc}
%   }
%   \subfloat[\small{IoU Accuracy}]
%   {
%   \includegraphics[width=.48\columnwidth]{iou_seg_acc}
%   \label{fig:iou_seg_acc}
%   }
%   %\vspace{-5pt}
%   \caption{Segmentation accuracy comparison between Original algorithms and accelerated algorithm.}
%   \label{fig:seg_acc}
%   %\vspace{-10pt}
% \end{figure}

%\paragraph{Object Segmentation} The second two columns in \Fig{fig:app_acc} show the segmentation accuracy between our \proj algorithms and their corresponding algorithms. Here, we show the overall accuracy of PointNet++ and DGCNN. \Fig{fig:overall_seg_acc} shows, we achieve \fixme{$0.1\%$} accuracy improvement on PointNet++ and \fixme{0.3\%} of accuracy loss on DGCNN. We also studies the IoU accuracy with a threshold of $70\%$, \proj achieve the same accuracy on PointNet++ and \fixme{0.7\%} accuracy loss on DGCNN. Interestingly, our \proj algorithm of PointNet++ has a better accuracy than original DNN algorithm on both overall accuracy and IoU accuracy. This shows that \proj framework can possibly have higher application accuracy while improvement runtime performance of some DNN algorithms simultaneously.

% \begin{figure}[t]
%   %\vspace{-10pt}
%   \centering
%   \includegraphics[width=.8\columnwidth]{detection_acc}
%   \caption{2D Detection accuracy (BEV) comparison between Original algorithms and accelerated algorithm.}
%   \label{fig:det_acc}
%   %\vspace{-10pt}
% \end{figure}

%\paragraph{Object Detection} The last column in \Fig{fig:app_acc} shows the comparison of detection accuracy between original algorithm and accelerated algorithm on F-PointNet++. Here, we show 2D detection accuracy on BEV. In KITTI dataset, it has three classes, cars, pedestrian, and cyclist. Each class also has three levels of difficulties in visibility, we only show the geometric mean here. Overall, our accelerated algorithm can achieve similar or even better accuracy than original pipeline. Our average accuracy (72.5\%) is even better than original pipeline (71.3\%). In particular, our algorithm accuracy on cyclist is significantly better than original pipeline by 4.7\%. The other two categories have slight 0.9\% (car) and 0.1\% (pedestrian) accuracy loss, comparing against the original algorithm.

\subsection{Results on GPU}
\label{sec:eval:gpu}

\begin{figure}
    \centering    \includegraphics[width=\columnwidth]{gpu_speedup_energy}
    \caption{Speedup and energy reduction of the delayed-aggregation algorithm and the limited version of the algorithm on the mobile Pascal GPU on TX2.}
    \label{fig:sw_speedup_energy}
\end{figure}

We first show that our delayed-aggregation algorithm readily achieves significant speedups on today's GPU \textit{without} hardware support. \Fig{fig:sw_speedup_energy} shows the speedup and energy reduction of \proj on the Pascal GPU on TX2.

As a comparison, we also show the results of a limited version of delayed-aggregation, where only the matrix-vector multiplication (MVM) part of an MLP is hoisted before aggregation (Ltd-\proj). The limited delayed-aggregation algorithm is inspired by certain Graph Neural Network (GNN) implementations such as GCN~\cite{gcnpytorch, fey2019pytorchgeo, wang2019deep} and GraphSage~\cite{graphsagetf}. Note that by hoisting only the MVM rather than the entire MLP, Ltd-\proj is precise since MVM is linear. We refer interested readers to the wiki page of our code repository~\cite{mesorasiwiki} for a detailed comparison between our delayed-aggregation and GNN's limited delayed-aggregation.

On average, \proj achieves $1.6\times$ speedup and 51.1\% energy reduction compared to the original algorithms. In comparison, the limited delayed-aggregation algorithm achieves only $1.3\times$ speedup and 28.3\% energy reduction. Directly comparing with Ltd-\proj, \proj has $1.3\times$ speedup and 25.9\% energy reduction. This is because the limited delay-aggregation, in order to be precise, could be applied to only the first MLP layer. By being approximate, \proj does not have this constraint and thus enables larger benefits; the accuracy loss could be recovered through fine-tuning (\Fig{fig:app_acc}). \proj has similar performance as Ltd-\proj on DGCNN (c), LDGCNN, and DensePoint, because these three networks have only one MLP layer per module.

%, comparing against limited \textsc{Mesorasi}algorithms. Limited \textsc{Mesorasi} means we use a limited form of delayed-aggregation that hoists only the MVM part of an MLP. the idea is inspired from GNNs~\cite{fey2019pytorchgeo}

Although delayed-aggregation allows neighbor search and feature extraction to be executed in parallel, and our implementation does exploit the concurrent kernel execution in CUDA, we find that neighbor search and feature extraction in actual executions are rarely overlapped. Further investigation shows that this is because the available resources on the Pascal GPU on TX2 are not sufficient to allow both kernels to execute concurrently. We expect the speedup to be even higher on more powerful mobile GPUs in the future.

Overall, networks in which feature computation contributes more heavily to the overall time, such as PointNet++ (c) and F-PointNet (\Fig{fig:motivation-dist}), have higher MAC operation reductions (\Fig{fig:overall_ops_red}), and thus have higher speedups and energy reductions. This confirms that the improvements are mainly attributed to optimizing the MLPs in feature computation.

%In particular, \proj can speedup algorithms, like PointNet++ (c) and F-PointNet++, up to \fixme{1.8$\times$} with over \fixme{$50\%$} energy reduction. We also found that the overall speedup has the similar trend as MAC ops reduction in \Fig{fig:overall_ops_red}. This shows that the major contributor is the reduction from MLP.

%In addition, our accelerated algorithm can relax the dependency between feature grouping in the frontend and MLP in the backend. This gives us more opportunities of parallelism. We believe that, \proj can achieve much higher speedup on a more powerful GPU platform.

\subsection{Speedup and Energy Reduction}
\label{sec:eval:res}

\begin{figure}[t]
\centering
\subfloat[Speedup. Higher is better.]{
	\label{fig:hw_speedup}	\includegraphics[width=\columnwidth]{hw_speedup} }
\\
\vspace{-5pt}
\subfloat[Normalized energy. Lower is better.]{
	\label{fig:hw_energy}
	\includegraphics[width=\columnwidth]{hw_energy} } 
%\vspace{-5pt}
\caption{Speedup and energy reduction of \sys{\proj-SW} and \sys{\proj-HW} over the baseline (GPU+NPU), which is twice as fast and consumes one-third of the energy compared to the GPU, indicating an optimized baseline to begin with.}
%\vspace{-15pt}
\label{fig:hw_speedup_energy}
\end{figure}

\proj also improves the performance and energy consumption of emerging mobile SoCs with a dedicated NPU. \Fig{fig:hw_speedup} and \Fig{fig:hw_energy} show the speedup and the normalized energy consumption of the two \proj variants over the NPU+GPU baseline, respectively.

\paragraph{Software} The delayed-aggregation algorithm alone without AU support, i.e., \sys{\proj-SW}, has a $1.3\times$ speedup and 22\% energy saving over the baseline. The main contributor of the improvements is optimizing the MLPs in feature computation. \Fig{fig:systolic_speedup} shows the speedups and energy savings of the delayed-aggregation algorithm on feature computation. On average, the feature computation time is reduced by $5.1\times$ and the energy consumption is reduced by 76.3\%.
%However, these performance improvements are not reflected in the overall performance gains.

The large speedup on feature computation does not translate to similar overall speedup, because feature computation time has already been significantly reduced by the NPU, leaving less room for improvement. In fact, our GPU+NPU baseline is about 1.8$\times$ faster (\Fig{fig:hw_speedup}) and consumes 70\% less energy compared to the GPU (\Fig{fig:hw_energy}). The increased workload of aggregation also adds to the overhead, leading to overall lower speedup and energy reduction than on GPU.

\paragraph{Hardware} With the AU hardware, \sys{\proj-HW} boosts the speedup to $1.9 \times$ (up to $3.6\times$) and reduces the energy consumption by 37.6\% (up to $92.9\%$). DGCNN (s) has the least speedup because it has the least aggregation time (\Fig{fig:runtime_dist}), thus benefiting the least from the AU hardware.

%Overall, on a much faster NPU+GPU system \sys{\proj-HW} can still achieve the same speedup (\fixme{$1.6\times$}) as on the GPU (\Sect{sec:eval:gpu}). The reason is that with both an NPU and a GPU, neighbor search and feature extraction can now be executed in parallel, making up for the ``loss'' on a stronger baseline.

\Fig{fig:perf_details} shows the speedup and energy reduction of aggregation over the baseline (which executes aggregation on the GPU). Overall, \sys{\proj-HW} reduces the aggregation time by $7.5\times$ and reduces the energy by 99.4\%. The huge improvements mainly come from using a small memory structure customized to the data access patterns in aggregation.

\begin{figure}[t]
  %\vspace{-10pt}
  \centering
  \captionsetup[subfigure]{width=0.5\columnwidth}
  \subfloat[\small{Feature computation.}]
  {
  \includegraphics[width=.48\columnwidth]{systolic_speedup}
  \label{fig:systolic_speedup}
  }
  \subfloat[\small{Aggregation.}]
  {
  \includegraphics[width=.48\columnwidth]{group_speedup}
  \label{fig:group_speedup}
  }
  %\vspace{-5pt}
  \caption{Speedup and energy savings on feature computation and aggregation.}
  \label{fig:perf_details}
  %\vspace{-10pt}
\end{figure}

On average, 27\% (max 29\%) of PFT buffer accesses are to serve previous bank conflicts. The total time spent on PFT buffer accesses is 1.5$\times$ of the ideal case without bank conflicts. Empirically we do not observe pathological cases.

The AU's speedup varies across networks. For instance, the speedup on PointNet++ (c) is over 3$\times$ higher than that of F-PointNet. This is because the speedup decreases as bank conflict increases; bank conflicts occur more often when neighbor search returns more neighbors. The neighbor searches in PointNet++ (c) mostly return 32 neighbors, whereas neighbor searches in F-PointNet return mostly 128 neighbors, significantly increasing the chances of bank conflicts. This also explains why PointNet++ (c) has overall higher speedup than F-PointNet (\Fig{fig:hw_speedup}).
%While DGCNN (s) has much higher aggregation speedup than F-PointNet, the overall speedup is much less significant because aggregation contributes much less to the overall time in DGCNN (s) (\Fig{fig:runtime_dist}).

\subsection{Results with Neighbor Search Engine (NSE)}
\label{sec:eval:nse}

From the evaluations above, it is clear that the improvements of \proj will ultimately be limited by the neighbor search overhead, which \proj does not optimize and becomes the ``Amdahl's law bottleneck.''
%The neighbor search bottleneck is particularly significant in networks where neighbor search time is significant, e.g., DGCNN (s) (\Fig{fig:motivation-dist}).

To assess the full potential of \proj, we evaluate it in a futuristic SoC that incorporates a dedicated neighbor search engine (NSE) that accelerates neighbor searches. We implement a recently published NSE built specifically for accelerating neighbor searches in point cloud algorithms~\cite{xu2019tigris}, and incorporate it into our SoC model. On average, the NSE provides over 60$\times$ speedup over the GPU. Note that the NSE is \textit{not} our contribution. Instead, we evaluate the potential speedup of \proj if an NSE is available.

The speedup of \proj greatly improves when neighbor search is no longer a bottleneck. \Fig{fig:nse_speedup} shows the speedups of \sys{\proj-SW} and \sys{\proj-HW} on the NSE-enabled SoC. On average, \sys{\proj-SW} achieves $2.1\times$ speedup and \sys{\proj-HW} achieves $6.7\times$ speedup. The two DGCNN networks have particularly high speedups because neighbor search contributes heavily to their execution times (\Fig{fig:motivation-dist}).

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{nse_speedup}
    \caption{\sys{\proj-SW} and \sys{\proj-HW} speedup over an NSE-enabled SoC (GPU+NPU+NSE), which is 4.0$\times$ faster than the GPU by accelerating both MLP and neighbor search.}
    \label{fig:nse_speedup}
\end{figure}

\subsection{Sensitivity Study}
\label{sec:eval:sen}

The evaluations so far are based on one hardware configuration. We now study how the improvements vary with different hardware resource provisions. In particular, we focus on two types of hardware resources: the baseline NPU and the AU augmentation. Due to the page limit, we show only the results of PointNet++ (s). The general trend holds.

%In our evaluation, we only explore one hardware setting. Here, we provide the extensive sensitivity analyses on varying configurations of NPU and AU. 

\paragraph{NPU} We find that \proj has higher speedups when the NPU is smaller. \Fig{fig:sa_profile} shows how the speedup and normalized energy of \sys{\proj-HW} over the baseline vary as the systolic array (SA) size increases from $8 \times 8$ to $48 \times 48$. As the SA size increases, the feature extraction time decreases, and thus leaving less room for performance improvement. As a result, the speedup decreases from 2.8$\times$ to 1.2$\times$.

Meanwhile, the energy reduction increases from 17.7\% to $23.4\%$. This is because a large SA is more likely throttled by memory bandwidth, leading to overall higher energy.

%The reason of decreasing overall speedup is that our pipeline can hide the latency of feature extraction completely, thus, more powerful NPU would only reduce the latency of baseline but not \proj. Meanwhile, we also observe the slight increase in speedup on feature extraction part.

\paragraph{AU} We find that the AU energy consumption is sensitive to the NIT and PFT buffer sizes. \Fig{fig:au_profile} shows the AU energy under different NIT and PFT buffer sizes. The results are normalized to the nominal design point described in \Sect{sec:exp} (i.e., a 64 KB of PFT and a 12 KB NIT).

The energy consumption increases as the PFT and NIT buffer sizes decrease. In an extremely small setting with an 8 KB PFT buffer and a 3 KB NIT buffer, the AU energy increases by 32$\times$, which leads to a 5.6\% overall energy increase. This is because a smaller PFT buffer leads to more PFT partitions, which increases NIT buffer energy since each NIT entry must be read once per partition. Meanwhile, a smaller NIT requires more DRAM accesses, whose energy dominates as the PFT buffer becomes very small. On the other extreme, using a 256 KB PFT buffer and a 96 KB NIT buffer reduces the overall energy by 2.0\% while increasing the area overhead by 4$\times$. Our design point balances energy saving and area overhead.


\begin{figure}[t]
\centering
\begin{minipage}[t]{0.48\columnwidth}
  \centering
  \includegraphics[width=\columnwidth]{systolic_profile}
  \caption{Sensitivity of the speedup and energy to the systolic array size.}
  \label{fig:sa_profile}
\end{minipage}
\hspace{2pt}
\begin{minipage}[t]{0.48\columnwidth}
  \centering
  \includegraphics[width=\columnwidth]{au_profile}
  \caption{Sensitivity of AU energy consumption to the NIT/PFT buffer sizes.}
  \label{fig:au_profile}
\end{minipage}
\end{figure}


==> Mesorasi_ Enabling Efficient Point Cloud Analytics via Delayed-Aggregation/exp.tex <==
\section{Experimental Setup}
\label{sec:exp}

%This section introduces the experimental setup in hardware and software.
%
%\subsection{Hardware Setup}
%\label{sec:exp:hw}

\paragraph{Hardware Implementation} We develop RTL implementations for the NPU and its augmentations for the aggregation unit (AU). The NPU is based on the systolic array architecture, and consists of a $16 \times 16$ PE array. Each PE consists of two input registers, a MAC unit with an accumulator register, and simple trivial control logic. This is identical to the PE in the TPU~\cite{jouppi2017datacenter}. Recall that MLPs in point cloud networks process batched inputs (\Fig{fig:baselinealgo}), so the MLPs perform matrix-matrix product that can be efficiently implemented on a systolic array. The NPU's global buffer is sized at 1.5 MB and is banked at a 128 KB granularity.

The PFT buffer in the AU is sized at 64 KB with 32 banks. The NIT buffer is doubled-buffered; each buffer is implemented as one SRAM bank sized at 12 KB and holds 128 entries. The NIT buffer produces one entry per cycle. Each entry is 98 Bytes, accommodating 64 neighbor indices (12 bits each). Each of the two shift registers is implemented as 256 flip-flops (4-byte each). The datapath mainly consists of 1) one 33-input max unit and 256 subtraction units in the reduction unit, and 2) 32 32-input MUXes in the AGU.
% Note: the 32 32-input MUXes in the AGU is basically the crossbar that routes (at most) 32 addresses to the 32 banks. Each bank is 2KB and word size is 4B, so each bank has 512 words, so the input address to each bank is 9-bit. So each MUX here is a 32-input 9-bit MUX. What we save is the crossbar that routes the data back fro the banks to the ports. There would also be 32 32-input MUX, but each input to the MUX would 32-bit, since each output of a bank is 1 word, i.e., 4 bytes.

The design is clocked at 1 GHz. The RTL is implemented using Synposys synthesis and Cadence layout tools in TSMC 16nm FinFET technology, with SRAMs generated by an Arm memory compiler. Power is simulated using Synopsys PrimeTimePX, with fully annotated switching activity.

%To evaluate the \proj SoC design, we build a simulator similar to GemDroid~\cite{chidambaram2014gemdroid}. 
\paragraph{Experimental Methodology} The latency and energy of the NPU (and its augmentation) are obtained from post-synthesis results of the RTL design. We model the GPU after the Pascal mobile GPU in the Nvidia Parker SoC hosted on the Jetson TX2 development board~\cite{tx2spec}. The SoC is fabricated in a 16 nm technology node, same as our NPU. We directly measure the GPU execution time as well as the kernel launch time. The GPU energy is directly measured using the built-in power sensing circuity on TX2.
%, which are faithfully incorporated into our SoC model

The DRAM parameters are modeled after Micron 16 Gb LPDDR3-1600 (4 channels) according to its datasheet~\cite{micronlpddr3}. DRAM energy is calculated using Micron's System Power Calculators~\cite{microdrampower} using the memory traffic, which includes: 1) GPU reading input point cloud, 2) NPU accessing MLP kernels and activations each layer, and 3) GPU writing NIT and NPU reading NIT. Overall, the DRAM energy per bit is about 70$\times$ of that of SRAM, matching prior work~\cite{Yazdanbakhsh2018GAN, gao2017tetris}.

The system energy is the aggregation of GPU, NPU, and DRAM. The overall latency is sum of GPU, NPU, and DRAM minus: 1) double buffering in the NPU, and 2) parallel execution between neighbor search on GPU and feature computation on NPU. Due to double-buffering, the overall latency is dominated by the compute latency, not memory.

%To evaluate the \proj SoC design, we build a cycle-level model similar to that in GemDroid~\cite{chidambaram2014gemdroid}. We capture the timing of the (augmented) NPU, GPU, and their interactions through the DRAM, from which we estimate the overall performance. The energy consumption is aggregated from that of individual components.

%We model the GPU after the Pascal mobile GPU in the Nvidia Parker SoC hosted on the Jetson TX2 development board~\cite{tx2spec}. The SoC is fabricated in a 16 nm technology node, same as our NPU. We directly measure the GPU execution time as well as the kernel launch time, which are faithfully incorporated into our SoC model. The GPU energy is directly measured using the built-in power sensing circuity on TX2. The off-chip DRAM energy is modeled after four Micron 16 Gb LPDDR3-1600 channels~\cite{micronlpddr3}, similar to that in TX2.

%\subsection{Software Setup}
%\label{sec:exp:sw}

\begin{table} 
\caption{Evaluation benchmarks.}
\resizebox{\columnwidth}{!}{
\renewcommand*{\arraystretch}{1}
\renewcommand*{\tabcolsep}{10pt}
\begin{tabular}{ cccc } 
\toprule[0.15em]
\textbf{\specialcell{Application\\Domains}} & \textbf{\specialcell{Algorithm}} & \textbf{Dataset} & \textbf{Year} \\ 
\midrule[0.05em]
\specialcell{Classification} &  \specialcell{PointNet++ (c)\\DGCNN (c)\\LDGCNN\\DensePoint} & ModelNet40 & \specialcell{2017\\2019\\2019\\2019} \\
\midrule[0.05em]
\specialcell{Segmentation} &  
\specialcell{PointNet++ (s)\\DGCNN (s)} & ShapeNet & \specialcell{2017\\2019} \\
\midrule[0.05em]
\specialcell{Detection} &  \specialcell{F-PointNet} & KITTI & \specialcell{2018} \\
\bottomrule[0.15em]
\end{tabular}
}
\label{tab:eval_app}
\end{table}

\paragraph{Software Setup} \Tbl{tab:eval_app} lists the point cloud networks we use, which cover different domains for point cloud analytics including object classification, segmentation, and detection. The networks cover both classic and recent ones (2019).

For classification, we use four networks: PointNet++~\cite{qi2017pointnet++}, DGCNN~\cite{wang2019dynamic}, LDGCNN~\cite{zhang2019linked}, and DensePoint~\cite{liu2019densepoint}; we use the ModelNet40~\cite{wu20153d} dataset. We report the standard overall accuracy metric. To evaluate segmentation, we use the variants of PointNet++ and DGCNN specifically built for segmentation, and use the ShapeNet dataset~\cite{shapenet2015}. We report the standard mean Intersection-over-Unit (mIoU) accuracy metric. Finally, we use F-PointNet~\cite{qi2018frustum} as the object detection network. We use the KITTI dataset~\cite{geiger2012we} and report the geometric mean of the IoU metric (BEV) across its classes.

%Note that although the segmentation and classification networks share the same structure, they have different internal implementations, as is evident in the very different execution times shown in \Fig{fig:motivation-dist}. We use the released TensorFlow implementations of these networks, and implement the delayed-aggregation versions of these networks in TensorFlow too.

We optimize the author-released open-source version of these networks to obtain stronger software baselines. We: 1) removed redundant data duplications introduced by \texttt{tf.tile}; 2) accelerated the CPU implementation of an important kernel, 3D Interpretation (\texttt{three\_interpolate}), with a GPU implementation; 3) replaced the Farthest Point Sampling with random sampling in PointNet++ with little accuracy loss; 4) replaced the Grouping operation (\texttt{group\_point}) with an optimized implementation (\texttt{tf.gather}) to improve the efficiency of grouping/aggregation. On TX2, our baseline networks are 2.2$\times$ faster than the open-source versions.

%\begin{itemize}
%    \item Object classification: we evaluate our framework on two different networks, Pointnet++\cite{} and DGCNN\cite{}.
%    \item Object segmentation: we evaluate our framework on two networks, Pointnet++\cite{} and DGCNN\cite{}.
%    \item Object detection: we evaluate our framework on one network, Frustum-PointNet-v2~\cite{}.
%\end{itemize}

%\paragraph{Object Classification} From autonomous driving to  drone and robot navigation, numerous applications use point clouds to recognize objects. Here we test two popular object classification DNNs, Pointnet++\cite{} and DGCNN\cite{}. To evaluate on these two algorithms, we use a dataset, ModelNet40~\cite{}. ModelNet40 dataset has total 12,311 CAD models and consists of 40 categories of point clouds generated from artificial CAD models. Each point cloud contains 1024 points. We report \fixme{average class accuracy} and \fixme{overall accuracy}in our evaluation.
%
%\paragraph{Object Segmentation} Understand an object in more details includes semantically segmenting the object into different parts. Object segmentation serves as another level of intelligence and foundation. We evaluate our framework on two different DNN algorithms, Pointnet++~\cite{} and DGCNN~\cite{}, using ShapeNet dataset~\cite{}. ShapeNet contains 16,881 shapes from 16 main categories, which are annotated with 50 different parts in total. Every point cloud contains 1024 points and has two to five parts and sampled points are labelled in ground truth. In our evaluation, we use two standard metrics, accuracy and mean IoU (mIoU). mIoU is calculated by averaging the IoU of all part types in one shape.
%
%\paragraph{Object Detection} Detecting different objects is critical to contiguous robot perception. Here, we choose F-Pointnet++~\cite{} as the DNN algorithm in object detection task and use KITTI dataset. KITTI dataset consists of 7481 training point clouds and 7518 test point clouds generated from RGB-D images. There are three main categories in KITTI dataset, car, cyclist and pedestrian. We use the widely adopted metric, Intersect-over-Union (IoU) score as
%a standard for object detection. Here, we set IoU threshold 0.7.

%\subsection{Evaluation Plan}
%\label{sec:exp:plan}

\paragraph{Baseline} We mainly compare with a generic NPU+GPU SoC without any \proj-related optimizations. Compared to the baseline, our proposal improves both the software, i.e., the delayed-aggregation algorithm as well as hardware, i.e., the aggregation unit (AU) augmentations to the NPU.

%We also compare with the mobile Pascal GPU on TX2 to demonstrate that the delayed-aggregation algorithm could readily achieve improvements on today's systems without hardware. To show the full potential of \proj, we also evaluate on a futuristic SoC

%We normalize the baseline and \proj's results (performance and energy numbers) to a pure GPU implementation of the original algorithm.

%We compare against two baselines. The first baseline is a Pascal mobile GPU in the 16 nm Nvidia Parker SoC hosted on the Jetson TX2 development board~\cite{??}. The entire point cloud networks, including neighbor search, aggregation, and feature extraction executes on the GPU. We will apply our delayed-aggregation algorithms, and demonstrate the benefits of a pure-software implementation of \proj.

%\fixme{One baseline hardware is the commodity TX2 platform, on which we run the existing point cloud algorithms and our new algorithms. Another baseline is our modeled SoC that has a NPU and a GPU. By comparing our NPU-enabled SoC with TX2, we establish that the former is better, and thus the rest of the evaluation will be using that as the hardware baseline. In other words, we want to show that using an NPU for executing the MLP layers are faster than executing everything on GPU.}

\paragraph{Variants} To decouple the contributions of our algorithm and hardware, we present two different \proj variants:
\begin{itemize}
    %\setlength\itemsep{-2pt}
    \item \sys{\proj-SW}: delayed-aggregation without AU support. Neighbor search and aggregation execute on the GPU; feature computation executes on the NPU.
    \item \sys{\proj-HW}: delayed-aggregation with AU support. Neighbor search executes on the GPU; aggregation and feature computation execute on the NPU.
\end{itemize}



==> Mesorasi_ Enabling Efficient Point Cloud Analytics via Delayed-Aggregation/intro.tex <==
\section{Introduction}
\label{sec:intro}

In recent years, we have seen the explosive rise of intelligent machines that operate on \textit{point clouds}, a fundamental visual data representation that provides a direct 3D measure of object geometry, rather than 2D projections (i.e., images). For instance, Waymo’s self-driving cars carry five LiDAR sensors to gather point clouds from the environment in order to estimate the trajectory over time and to sense object depths~\cite{waymolidar}. Augmented Reality (AR) development frameworks such as Google's ARCore enable processing point clouds for localization (SLAM) and scene understanding~\cite{arcore}. While point cloud algorithms traditionally use ``hand-crafted'' features~\cite{rusu2009fast, tombari2010unique}, they are increasingly moving towards learned features using deep learning~\cite{qi2017pointnet++, wang2019dynamic}, which poses significant efficiency challenges.

We present \proj\footnote{\textipa{[me-s"@ra-z\=e]} Between two vision modes. \textit{meso}-: in the middle; from Ancient Greek \textmu$\acute{\varepsilon}$\textsigma\textomikron\textvarsigma. \textit{orasi}: vision; from Greek $\acute{o}$\textrho\textalpha\textsigma\texteta.}, an algorithm-architecture co-designed system that simultaneously improves the performance and energy efficiency of point cloud algorithms without hurting the accuracy. \proj applies algorithmic and architectural optimizations that exploit characteristics unique to point cloud. Critically, our algorithmic optimizations can directly benefit software running on commodity GPUs without hardware support. Minor augmentations to contemporary DNN accelerators (NPU) unlock further improvements, widening the applicability of \proj.

%While conventional image and video analytics algorithms have been well-optimized, point cloud analytics requires considerably different algorithms that are inefficient on today's hardware. 

We start by understanding the characteristics of point cloud algorithms. They inherit the key idea of conventional image/video processing algorithms (e.g., CNNs): extracting features from local windows (neighborhoods) iteratively and hierarchically until the final output is calculated. However, since points in a point cloud are arbitrarily spread in the 3D space, point cloud algorithms require explicit neighbor search and point aggregation operations (as opposed to direct memory indexing) before the actual feature computation.

This leads to two fundamental inefficiencies. First, the three key steps---neighbor search, aggregation, and feature computation---are serialized, leading to long critical path latency. In particular, neighbor search and feature computation dominate the execution time. Second, feature computation operates on aggregated neighbor points, which are inherently redundant representations of the original points, leading to massive memory and computation redundancies.

We propose \textit{delayed-aggregation}, a new algorithmic primitive for building efficient point cloud networks. The key idea is to delay aggregation after feature computation by exploiting the \textit{approximately distributive} property of feature computation over aggregation. In this way, feature computation operates directly on original input points rather aggregated neighbors, significantly reducing the compute cost and memory accesses. In addition, delayed-aggregation breaks the serialized execution chain in existing algorithms, overlapping neighbor search and feature computation---the two performance bottlenecks---to hide long latencies.

To maximize the benefits of delayed-aggregation, we propose minor extensions to conventional DNN accelerators. We find that delayed-aggregation increases the overhead of aggregation, which involves irregular gather operations. The hardware extension co-designs an intelligent data structure partitioning strategy with a small but specialized memory unit to enable efficient aggregation. Our hardware extensions are integrated into generic DNN accelerators without affecting the rest of a mobile Systems-on-a-Chip (SoC).

We evaluate \proj on a set of popular point cloud algorithms and datasets. On the mobile Pascal GPU on TX2, a representative mobile platform today, the delayed-aggregation algorithm alone without hardware support achieves 1.6$\times$ speedup and 51.1\% energy reduction while retaining the accuracy (-0.9\% loss to 1.2\% gains). We implement and synthesize the \proj hardware support in a 16nm process node and integrate it into a state-of-the-art SoC that incorporates a GPU and an NPU. With 3.8\% area overhead to the NPU (\textless 0.05\% of a typical SoC area), \proj achieves up to 3.6$\times$ speedup, which increases to 6.7 on a futuristic SoC with a dedicated neighbor search accelerator.

The artifact is publicly available at \url{https://github.com/horizon-research/efficient-deep-learning-for-point-clouds}. In summary, this paper makes the following contributions:

\begin{itemize}
    %\setlength\itemsep{-1pt}
	\item We comprehensively characterize the performance bottlenecks as well as the memory and compute cost of state-of-the-art point cloud algorithms, and identify the root-causes of the algorithmic inefficiencies.
	\item We propose delayed-aggregation, an efficient algorithm primitive that enables point cloud algorithms to hide the performance bottlenecks and to reduce the overall workload. Delayed-aggregation can readily achieve significant speedup and energy savings on current-generation mobile GPUs without hardware modification.
	\item We co-design hardware with delayed-aggregation to achieve even greater speedups with minor, yet principled, augmentations to conventional DNN accelerators while retaining the modularity of existing SoCs.
\end{itemize}


























==> Mesorasi_ Enabling Efficient Point Cloud Analytics via Delayed-Aggregation/macros.tex <==
%!TEX root=paper.tex

\newcommand{\website}[1]{{\tt #1}}
\newcommand{\program}[1]{{\tt #1}}
\newcommand{\benchmark}[1]{{\it #1}}
\newcommand{\fixme}[1]{{\textcolor{red}{\textit{#1}}}}

\newcommand*\circled[2]{\tikz[baseline=(char.base)]{
            \node[shape=circle,fill=black,inner sep=1pt] (char) {\textcolor{#1}{{\footnotesize #2}}};}}

\ifx\figurename\undefined \def\figurename{Figure}\fi
\renewcommand{\figurename}{Fig.}
\renewcommand{\paragraph}[1]{\textbf{#1} }
\newcommand{\figline}{{\vspace*{.05in}\hline}}

\newcommand{\Sect}[1]{Sec.~\ref{#1}}
\newcommand{\Fig}[1]{Fig.~\ref{#1}}
\newcommand{\Tbl}[1]{Tbl.~\ref{#1}}
\newcommand{\Equ}[1]{Equ.~\ref{#1}}
\newcommand{\Apx}[1]{Apdx.~\ref{#1}}
\newcommand{\Alg}[1]{Algo.~\ref{#1}}

\newcommand{\specialcell}[2][c]{\begin{tabular}[#1]{@{}c@{}}#2\end{tabular}}
\newcommand{\note}[1]{\textcolor{red}{#1}}

\newcommand{\proj}{\textsc{Mesorasi}\xspace}
\newcommand{\mode}[1]{\underline{\textsc{#1}}\xspace}
\newcommand{\sys}[1]{\underline{\textsc{#1}}}

\newcommand{\no}[1]{#1}
\renewcommand{\no}[1]{}
\newcommand{\RNum}[1]{\uppercase\expandafter{\romannumeral #1\relax}}

\def\cA{{\mathcal{A}}}
\def\cF{{\mathcal{F}}}
\def\cN{{\mathcal{N}}}

% checkmark and xmark in the pifont package
%\newcommand{\cmark}{\ding{51}}
%\newcommand{\xmark}{\ding{55}}


==> Mesorasi_ Enabling Efficient Point Cloud Analytics via Delayed-Aggregation/motivation.tex <==
\section{Motivation}
\label{sec:mot}

We first introduce the general flow of point cloud algorithms and identify key operators (\Sect{sec:mot:conv}). We then characterize point cloud algorithms on today's hardware systems to understand the algorithmic and execution bottlenecks (\Sect{sec:mot:char}), which motivate the \proj design.

\begin{figure}[t]
    \centering
    \subfloat[Network architecture of PointNet++~\cite{qi2017pointnet++}.]{
      \label{fig:pointnet2}
      \includegraphics[width=\columnwidth]{module-pointnet2}
    }
    \\
    \subfloat[DGCNN~\cite{wang2019dynamic} network architecture. ``\textbf{+}'' is tensor concatenation.]{
      \label{fig:dgcnn}
      \includegraphics[width=\columnwidth]{module-dgcnn}
    }
    %\vspace{-5pt}
    \caption{Point cloud networks consist of a set of modules, which extract local features from the input point cloud iteratively and hierarchically to calculate the final output.}
    \label{fig:module}
\end{figure}

\begin{figure}[t]
%\vspace{-5pt}
\centering
\subfloat[Convolution in conventional CNNs can be thought of as two steps: 1) neighbor search ($\cN$) by directly indexing adjacent pixels and 2) feature computation ($\cF$) by a dot product.]
{
  \includegraphics[trim=0 0 0 0, clip, width=\columnwidth]{convreuse}
  \label{fig:convreuse}
}
\\
\subfloat[Point cloud networks consist of three main steps: neighbor search ($\cN$), aggregation ($\cA$), and feature computation ($\cF$). $\cN$ requires an explicit neighbor search; $\cA$ normalizes neighbors to their centroid; $\cF$ is an MLP with batched inputs (i.e., shared MLP weights).]
{
  \includegraphics[trim=0 0 0 0, clip, width=\columnwidth]{nsreuse}
  \label{fig:nsreuse}
}
%\vspace{-5pt}
\caption{Comparing a convolution layer in conventional CNNs and a module in point cloud networks.}
\label{fig:conv}
%\vspace{-15pt}
\end{figure}

\begin{figure*}[t]
\centering
\includegraphics[width=2.1\columnwidth]{baselinealgo}
%\vspace{-5pt}
\caption{The first module in PointNet++~\cite{qi2017pointnet++}. The same MLP is shared across all the row vectors in a Neighbor Feature Matrix (NFM) and also across different NFMs. Thus, MLPs in point cloud networks process batched inputs, effectively performing matrix-matrix multiplications. The (shared) MLP weights are small in size, but the MLP activations are much larger. This is because the same input point is normalized to different values in different neighborhoods before entering the MLP. For instance, \texttt{P3} is normalized to different offsets with respect to \texttt{\underline{P1}} and \texttt{\underline{P2}} as \texttt{P3} is a neighbor of both \texttt{\underline{P1}} and \texttt{\underline{P2}}. In point cloud algorithms, most points are normalized to 20 to 100 centroids, proportionally increasing the MLP activation size.}
\label{fig:baselinealgo}
\end{figure*}

\subsection{Point Cloud Network Architecture}
\label{sec:mot:conv}

\paragraph{Module} The key component in point cloud algorithms is a \textit{module}. Each module transforms an input point cloud to an output point cloud, similar to how a convolution \textit{layer} transforms an input feature map to an output feature map in conventional CNNs. A point cloud network assembles different modules along with other common primitives such as fully-connected (FC) layers. \Fig{fig:pointnet2} and \Fig{fig:dgcnn} illustrate the architecture of two representative point cloud networks, PointNet++~\cite{qi2017pointnet++} and DGCNN~\cite{wang2019dynamic}, respectively.

\paragraph{Module Internals} Each point $\mathbf{p}$ in a point cloud is represented by a feature vector, which in the original point cloud is simply the 3D coordinates of the point. The input point cloud to a module is represented by an $N_{in} \times M_{in}$ matrix, where $N_{in}$ denotes the number of input points and $M_{in}$ denotes the input feature dimension. Similarly, the output point cloud is represented by an $N_{out} \times M_{out}$ matrix, where $N_{out}$ denotes the number of output points and $M_{out}$ denotes the output feature dimension. Note that $N_{in}$ and $N_{out}$ need not be the same; neither do $M_{in}$ and $M_{out}$.

%The input (output) feature dimensions could be thought of as the input (output) channel depth. Just as the input image to the first convolution layer has three channels (i.e., R, G, and B colors), the input point cloud to the first module has a three dimension feature vector (i.e., <$x, y, z$> coordinates).

%The Convolution layers function as feature transformations. In 3-d point networks, both the input and output are point sets, in which each point has its feature vector. In general, the Convolution layer can be expressed in formula: $P_{out} = Convolution(P_{in})$, where $P_{in}$ is the input and $P_{out}$ the output. In 3-d point cloud networks, the input Point Cloud is represented by a $N \times M_{in}$ matrix, where $N$ denotes the number of points and $M_{in}$ the dimension of each feature vector. Similarly, $P_{out}$ is a $N \times M_{out}$ matrix. Notice that $M_{out}$ is independent of $M_{in}$, they can be the same or different.

Internally, each module extracts local features from the input point cloud. This is achieved by iteratively operating on a small \textit{neighborhood} of input points, similar to how a convolution layer extracts local features of the input image through a sliding window. \Fig{fig:conv} illustrates this analogy.

Specifically, each output point $\mathbf{p}_o$ is computed from an input point $\mathbf{p}_i$ in three steps --- neighbor search ($\cN$), aggregation ($\cA$), and feature computation ($\cF$):
\begin{align}
  \mathbf{p}_o = \cF(\cA(\cN(\mathbf{p}_i),~~\mathbf{p}_i))
\end{align}
\noindent where $\cN$ returns $K$ neighbors of $\mathbf{p}_i$, $\cA$ aggregates the $K$ neighbors, and $\cF$ operates on the aggregation ($\mathbf{p}_i$ and its $K$ neighbors) to generate the output $\mathbf{p}_o$.

The same formulation applies to the convolution operation in conventional CNNs as well, as illustrated in \Fig{fig:conv}. However, the specifics of the three operations differ in point cloud networks and CNNs. Understanding the differences is key to identifying optimization opportunities.

\paragraph{Neighbor Search} $\cN$ in convolution returns $K$ adjacent pixels in a regular 3D tensor by simply \textit{indexing} the input feature map ($K$ dictated by the convolution kernel volume). In contrast, $\cN$ in point cloud networks requires explicit \textit{neighbor search} to return the $K$ nearest neighbors of $\mathbf{p}_i$, because the points are irregularly scattered in the space. Similar to the notion of a ``stride'' in convolution, the neighbor search might be applied to only a subset of the input points, in which case $N_{out}$ would be smaller than $N_{in}$, as is the case in \Fig{fig:nsreuse}.

%, which sometimes is approximated by $K$ arbitrary points within certain range to reduce the search cost

% This is because CNNs operate on regular tensors, in which the neighbors of any pixel <$x, y, z$> on a 2-d image, its neighbors are known statically as long as the stencil window size of convolutions is given. However, for 3-d point clouds, $N$ is a non-trivial operation that requires heavy distance calculation.

\paragraph{Aggregation} Given the $K$ pixels, convolution in CNNs directly operates on the raw pixel values. Thus, conventional convolution skips the aggregation step.

In contrast, point cloud modules operate on the \textit{relative} value of each point in order to correlate a neighbor with its centroid. For instance, a point $\mathbf{p}_3$ could be a neighbor of two centroids $\mathbf{p}_1$ and $\mathbf{p}_2$ (as is the case in \Fig{fig:nsreuse}). To differentiate the different contributions of $\mathbf{p}_3$ to $\mathbf{p}_1$ and $\mathbf{p}_2$, $\mathbf{p}_3$ is \textit{normalized} to the two centroids by calculating the offsets $\mathbf{p}_3 - \mathbf{p}_1$ and $\mathbf{p}_3 - \mathbf{p}_2$ for subsequent computations.

Generally, for each neighbor $\mathbf{p}_k \in \cN(\mathbf{p}_i)$, the aggregation operation calculates the offset $\mathbf{p}_k - \mathbf{p}_i$ (a $1 \times M_{in}$ vector). All $K$ neighbors' offsets form a Neighbor Feature Matrix (NFM) of size $K \times M_{in}$, effectively aggregating the neighbors of $\mathbf{p}_i$.

\begin{figure*}[t]
\centering
\begin{minipage}[t]{0.48\columnwidth}
  \centering
  \includegraphics[trim=0 0 0 0, clip, height=1.40in]{motivation-exe-time}
  \caption{Latency of five point cloud networks on the Pascal GPU on TX2. Results are averaged over 100 executions, and the error bars denote one standard deviation.}
  \label{fig:motivation-exe-time}
\end{minipage}
\hspace{5pt}
\begin{minipage}[t]{0.48\columnwidth}
  \centering
  \includegraphics[trim=0 0 0 0, clip, height=1.40in]{motivation-dist}
  \caption{Time distribution across the three main point cloud operations ($\cN$, $\cA$, and $\cF$). The data is averaged on the mobile Pascal GPU on TX2 over 100 executions.}
  \label{fig:motivation-dist}
\end{minipage}
\hspace{5pt}
\begin{minipage}[t]{0.42\columnwidth}
  \centering
  \includegraphics[trim=0 0 0 0, clip, height=1.45in]{motivation-pts-use}
  \caption{Distribution of the number of points ($y$-axis) that occur in a certain number of neighborhoods ($x$-axis). We profile 32 inputs (curves).}
  \label{fig:motivation-pts-use}
\end{minipage}
\hspace{5pt}
\begin{minipage}[t]{0.55\columnwidth}
  \centering
  \includegraphics[trim=0 0 0 0, clip, height=1.40in]{mac_ops}
  \caption{MAC operation comparison between point cloud networks (130K input points per frame~\cite{geiger2012we}) and conventional CNNs (nearly 130K pixels per frame).}
  \label{fig:motivation-mac}
\end{minipage}
\vspace{-5pt}
\end{figure*}

\paragraph{Feature Computation} $\cF$ in convolution is a dot product between the pixel values in a window and the kernel weights. In contrast,  $\cF$ in point cloud applies a multilayer perceptron (MLP) to each row vector in the NFM. Critically, all $K$ row vectors share the same MLP; thus, the $K$ input vectors are batched into a matrix and the MLP becomes a matrix-matrix product, transforming a $K \times M_{in}$ matrix to a $K \times M_{out}$ matrix.
%It is usually the case that all the Neighbor Feature Matrices share the same MLP.

In the end, a reduction operation then reduces the $K \times M_{out}$ matrix to a $1 \times M_{out}$ vector, which becomes the feature vector of an output point. A common choice for reduction is to, for each column independently, take the max of the $K$ rows.

\paragraph{Example} \Fig{fig:baselinealgo} shows the first module in PointNet++~\cite{qi2017pointnet++}, a classic point cloud network that many other networks build upon. This module transforms a point cloud with 1024 ($N_{in}$) points, each with a 3-D ($M_{in}$) feature vector, to a point cloud with 512 ($N_{out}$) points, each with an 128-D ($M_{out}$) feature vector, indicating that the neighbor search is applied to only 512 input points. Each neighbor search returns 32 ($K$) neighbors and forms a $32 \times 3$ NFM, which is processed by a MLP with 3 layers to generate a $32 \times 128$ matrix, which in turn is reduced to a $1 \times 128$ feature vector for an output point. In this particular network, all the NFMs also share the same MLP.

Note that while feature computation is not always MLP and normalization is not always differencing from centroids, they are the most widely used, both in classic networks (e.g., PointNet++~\mbox{\cite{qi2017pointnet++}}) and recent ones (e.g., DGCNN~\mbox{\cite{wang2019dynamic}}).

\subsection{Performance Characterizations}
\label{sec:mot:char}

We characterize point cloud networks on today's systems to understand the bottlenecks and optimization opportunities. To that end, we profile the performance of five popular point cloud networks on the mobile Pascal GPU on the Jetson TX2 development board~\cite{tx2spec}, which is representative of state-of-the-art mobile computing platforms. Please refer to \Sect{sec:exp} for a detailed experimental setup.
 
\paragraph{Time Distribution} \Fig{fig:motivation-exe-time} shows the execution times of the five networks, which range from 71 $ms$ to 5,200 $ms$, clearly infeasible for real-time deployment. The time would scale proportionally as the input size grows.
%For instance, for the fastest network PointNet++ (c), the latency would increase from 71 $ms$ to 530 $ms$ when the input size becomes 8$\times$ larger.

\Fig{fig:motivation-dist} further decomposes the execution time into the three components, i.e., Neighbor Search ($\cN$), Aggregation ($\cA$), and Feature Computation ($\cF$). $\cN$ and $\cF$ are the major performance bottlenecks. While $\cF$ consists of MLP operations that are well-optimized, $\cN$ (and $\cA$) is uniquely introduced in point cloud networks. Even if $\cF$ could be further accelerated on a DNN accelerator, $\cN$ has compute and data access patterns different from matrix multiplications~\cite{xu2019tigris}, and thus does not fit on a DNN accelerator.

Critically, $\cN$, $\cA$, and $\cF$ are serialized. Thus, they all contribute to the critical path latency; optimizing one alone would not lead to universal speedups. The serialization is inherent to today's point cloud algorithms: in order to extract local features of a point ($\cF$), the point must be aggregated with its neighbors ($\cA$), which in turn requires neighbor search ($\cN$). \proj's algorithm breaks this serialized execution chain, allowing $\cF$ and $\cN$ to be overlapped.

\paragraph{Memory Analysis} Point cloud networks have large memory footprints. While the MLP weights are small and are shared across input NFMs (\Fig{fig:baselinealgo}), the intermediate (inter-layer) activations in the MLP are excessive in size.
%This is because feature extraction operates on \textit{aggregated} neighbor points, forgoing the reuse opportunities inherent in point cloud data.

The ``Original'' category in \Fig{fig:layer_mem_red} shows the distribution of each MLP layer's output size across the five networks. The data is shown as a violin plot, where the high and low ticks represent the largest and smallest layer output size, respectively, and the width of the violin represents the density at a particular size value ($y$-axis). The layer output usually exceeds 2 MB, and could be as large as 32 MB, much greater than a typical on-chip memory size in today's mobile GPUs or DNN accelerators. The large activation sizes would lead to frequent DRAM accesses and high energy consumption.

% Fundamentally, the reason for the large activation sizes is that today's algorithms fail to exploit the reuse opportunities inherent in point cloud data. Specifically, points in overlapped neighborhoods are not reused in feature computation. 

%On average, each single point can be transformed into $K$ offsets (each offset is at the same size as a point), where $K$ is the size of each neighborhood. As the data size scales by $K$ times, what is worse is that there is no data reuse at all.
The large activation size is fundamental to point cloud algorithms. This is because an input point usually belongs to many overlapped neighborhoods, and thus must be normalized to different values, one for each neighborhood. \Fig{fig:nsreuse} shows a concrete example, where \texttt{P3} is a neighbor of both \texttt{P1} and \texttt{P2}; the aggregation operation normalizes \texttt{P3} to \texttt{P1} and \texttt{P2}, leading to two different relative values (\texttt{P3} - \texttt{P1} and \texttt{P3} - \texttt{P2}) that participate in feature computation, increasing the activation size. This is in contrast to convolutions, where pixels in overlapped neighborhoods (windows) are directly reused in feature computation (e.g., \texttt{P4} in \Fig{fig:convreuse}).

\begin{figure*}[t]
\centering
\includegraphics[width=2.1\columnwidth]{newalgo}
%\vspace{-5pt}
\caption{The delayed-aggregation algorithm applied to the first module in PointNet++. The MLP and neighbor search are executed in parallel, effectively delaying aggregation after feature computation. The input size of the MLP is much smaller (input point cloud as opposed to the aggregated NFMs), which significantly reduces the MAC operations and the intermediate activation sizes. Aggregation now operates on the output feature space (128-D in this case), whereas it previously operates on the input feature space (3-D in this case). Thus, the aggregation time increases and emerges as a new performance bottleneck.}
\label{fig:newalgo}
\end{figure*}

We use two networks, DGCNN~\cite{qi2017pointnet++} and PointNet++~\cite{ wang2019dynamic}, to explain the large activation sizes. \Fig{fig:motivation-pts-use} shows the distribution of the number of neighborhoods each point is in. Each curve corresponds to an input point cloud, and each ($x$, $y$) point on a curve denotes the number of points ($y$) that occur in a certain number of neighborhoods ($x$). In PointNet++, over half occur in more than 30 neighborhoods; in DGCNN, over half occurs in 20 neighborhoods. Since the same point is normalized to different values in different neighborhoods, this bloats the MLP's intermediate activations.
%For example, (20, 250) means that there are 250 points, each occurring in 20 neighborhoods. 

\paragraph{Compute Cost} The large activations lead to high multiply-and-accumulate (MACs) operations. \Fig{fig:motivation-mac} compares the number of MAC operations in three classic CNNs with that in the feature computation of point cloud networks. To use the same ``resolution'' for a fair comparison, the input point cloud has 130,000 points (e.g., from the widely-used KITTI Odometry dataset~\cite{geiger2012we}) and the CNN input has a similar amount of pixels. In feature computation alone, point cloud networks have an order of magnitude higher MAC counts than conventional CNNs. \proj's algorithm reduces both the memory accesses and MAC counts in feature computation.

\paragraph{Summary} Today's point cloud algorithms extract local features of a point by aggregating the point with its neighbors. The aggregation happens \textit{before} feature computation, which leads to two fundamental inefficiencies:

\begin{itemize}
    %\setlength\itemsep{-2pt}
	\item The two major performance bottlenecks, neighbor search and feature computation, are serialized.
	\item Feature computation operates on aggregated neighbor points, leading to high memory and compute cost.
\end{itemize}


==> Mesorasi_ Enabling Efficient Point Cloud Analytics via Delayed-Aggregation/related.tex <==
\section{Related Work}
\label{sec:related}

\paragraph{Point Cloud Analytics} Point cloud has only recently received extensive interests. Unlike conventional image/video analytics, point cloud analytics requires considerably different algorithms due to the unique characteristics of point cloud data. Most of the recent work focuses on the accuracy, exploring not only different data representation (e.g., 2D projection~\cite{qi2016volumetric}, voxelization~\cite{wu20153d, riegler2017octnet}, and raw points~\cite{qi2017pointnet++, wang2019dynamic}), but also different ways to extract features from points~\cite{simonovsky2017dynamic, wu2019pointconv, qi2017pointnet++, wang2019dynamic}. Our delayed-aggregation primitive can be thought of as a new, and efficient, way of extracting features from raw points.

\proj focuses on improving the efficiency of point cloud algorithms while retaining the high accuracy. In the same vein, PVCNN~\cite{liu2019point} combines point-based and voxel-based data representations in order to boost compute and memory efficiency. Different but complementary, \proj focuses on point-based neural networks. While PVCNN is demonstrated on GPUs, \proj not only directly benefits commodity GPUs, but also incorporates systematic hardware support that improves DNN accelerators.

Prior work has also extensively studied systems and architectures for accelerating neighbor search on GPU~\cite{Qiu2009GPU, Gieseke2014Buffer}, FPGA~\cite{Winterstein2013FPGA, Kuhara2013An, Heinzle2008A}, and ASIC~\cite{xu2019tigris}. Neighbor search contributes non-trivial execution time to point cloud networks. \proj hides, rather than reduces, the neighbor search latency, and directly benefits from faster neighbor search.

\paragraph{GNNs} Point cloud applications bear some resemblance to GNNs. After all, both deal with spatial/geometric data. In fact, some point cloud applications are implemented using GNNs, e.g., DGCNN~\cite{wang2019dynamic}.

However, existing GNN accelerators, e.g., HyGCN~\cite{yan2020hygcn}, are insufficient in accelerating point cloud applications. Fundamentally, GNN does not require explicit neighbor search (as a vertex's neighbors are explicitly encoded), but neighbor search is a critical bottleneck of all point cloud applications, as points are arbitrarily spread in 3D space. Our design hides the neighbor search latency, which existing GNN accelerators simply do not optimize for. In addition, \proj minimally extends conventional DNN accelerators instead of being a new accelerator design, broadening its applicability in practice.

From \Fig{fig:motivation-dist}, one might notice that $\cA$ in point cloud networks is much faster than $\cF$, which is the opposite in many GNNs~\cite{yan2020hygcn}. This is because $\cF$ in point cloud applications does much more work than $\cA$, opposite to GNNs. In point cloud application, $\cA$ simply gathers neighbor feature vectors, and $\cF$ operates on neighbor feature vectors (MLP on each vector). In contrast, $\cA$ in GNNs gathers and reduces neighbor feature vectors to one vector, and $\cF$ operates on the reduced vector (MLP on one vector).

%lots of HyGCN’s effort is spent, rightfully so, on optimizing for sparse graphs, which is not an issue for point clouds, which are stored in a dense representation. Finally, 

\paragraph{Domain-Specific Accelerator} Complementary to improving generic DNN accelerators, much of recent work has focused on improving the DNN accelerators for specific application domains such as real-time computer vision~\cite{buckler2018eva2, feng2019asv, zhu2018euphrates}, computational imaging~\cite{huang2019ecnn, mahmoud2018diffy}, and language processing~\cite{riera2018computation}. The NPU in the \proj architecture is a DNN accelerator specialized to point cloud processing. \proj also extends beyond prior visual accelerators that deal with 2D data (images and videos)~\cite{mahmoud2017ideal, leng2019energy, zhang2017race, mazumdar2017exploring, zhang2019distilling, dejaview} to 3D point clouds.

To keep the modularity of existing SoCs, \proj relies on the DRAM for inter-accelerator communication. That said, \proj could benefit from more direct accelerator communication schemes such as VIP~\cite{nachiappan2016vip} and Short-circuiting~\cite{yedlapalli2014short}. For instance, the NIT could be directly communicated to the NIT buffer from the GPU through a dedicated on-chip link, pipelining neighbor search with aggregation.

%One of our design principles is to keep the modularity of existing SoCs as much as possible. Therefore, our architectural augmentations are restricted to only the NPU, leaving other accelerators (e.g., the GPU or the NSE if available) unmodified.

%Nevertheless, in a custom-designed SoC it is possible to closely integrate the GPU/NSE with the NPU to improve the efficiency. For instance, the NIT could be directly transferred to the NIT buffer in the NPU through a dedicated on-chip link~\cite{??}. In this way, aggregation and neighbor search could be pipelined, in that whenever an entry is pushed into the NIT buffer the aggregation operation is triggered, potentially reducing the overall latency.

%Nachiappan et al. propose to coordinate the DVFS decision across different SoC IPs to improve the energy-efficiency of mobile applications~\cite{domainknowledge}. VIP proposes to streamline the data communication across different IP blocks to reduce memory traffic~\cite{vip}.

